Query-Efficient Algorithm to Find all Nash Equilibria in a Two-Player Zero-Sum Matrix Game

We study the query complexity of finding the set of all Nash equilibria $\mathcal X_\star \times \mathcal Y_\star$ in two-player zero-sum matrix games. Fearnley and Savani (2016) showed that for any randomized algorithm, there exists an $n \times n$ input matrix where it needs to query $\Omega(n^2)$ entries in expectation to compute a single Nash equilibrium. On the other hand, Bienstock et al. (1991) showed that there is a special class of matrices for which one can query $O(n)$ entries and compute its set of all Nash equilibria. However, these results do not fully characterize the query complexity of finding the set of all Nash equilibria in two-player zero-sum matrix games. In this work, we characterize the query complexity of finding the set of all Nash equilibria $\mathcal X_\star \times \mathcal Y_\star$ in terms of the number of rows $n$ of the input matrix $A \in \mathbb{R}^{n \times n}$, row support size $k_1 := |\bigcup_{x \in \mathcal X_\star} \text{supp}(x)|$, and column support size $k_2 := |\bigcup_{y \in \mathcal Y_\star} \text{supp}(y)|$. We design a simple yet non-trivial randomized algorithm that, with probability $1 - \delta$, returns the set of all Nash equilibria $\mathcal X_\star \times \mathcal Y_\star$ by querying at most $O(nk^5 \cdot \text{polylog}(n / \delta))$ entries of the input matrix $A \in \mathbb{R}^{n \times n}$, where $k := \max\{k_1, k_2\}$. This upper bound is tight up to a factor of $\text{poly}(k)$, as we show that for any randomized algorithm, there exists an $n \times n$ input matrix with $\min\{k_1, k_2\} = 1$, for which it needs to query $\Omega(nk)$ entries in expectation in order to find the set of all Nash equilibria $\mathcal X_\star \times \mathcal Y_\star$.

==> extra.tex <==
\textcolor{red}{Old algo.Ignore.}
\section{Extra old algo}
In this section, we describe $\textsc{Basic}$, a randomized algorithm that finds the set of all basic solutions. The key steps of this algorithm  is similar to the algorithm for finding the unique Nash equilibrium in \Cref{section:random:msne}.  We first begin with stating the guarantees of our randomized algorithm.

\begin{theorem}\label{thm:alg-multiple-ne}
Consider a matrix game $A\in\bbR^{n\times n}$. Let $k:=\max\{|\calX_\star|,|\calY_\star|\}$.
There is a randomized algorithm that with probability at least $1-\delta$ queries at most $O(nk^5\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of $A$ and finds all the basic solutions. 
\end{theorem}

Recall that each basic solution is a PSNE and it belongs to the set $\{(x,y):x\in \calX_\star,y\in\calY_\star\}$.
Let us assume that we know the values of $k_1:=|\calX_\star|$ and $k_2:=|\calY_\star|$. Towards the end of this section, we relax this assumption. 

\textbf{Description of the randomized procedure } \textsc{Basic}$(A,k_1,k_2)$:
Let $A\in\bbR^{n\times n}$ be the input matrix. Let $\bar M=\frac{1}{k_1k_2}\sum_{i=1}^{k_1}\sum_{j=1}^{k_2}M_{i,j}$ denote the average of entry-values of $M\in\mathbb{R}^{k_1\times k_2}$.
We construct a matrix $A^{(k_1,k_2)}\in \bbR^{\binom{n}{k_1} \times \binom{n}{k_2}}$ as follows.
First, we create two bijections $f_1:\binom{n}{k_1}\rightarrow \binom{[n]}{k_1}$ and $f_2:\binom{n}{k_2}\rightarrow \binom{[n]}{k_2}$.
Let $A^{(k_1,k_2)}_{i,j}=\bar M$ where $M$ is the sub-matrix of $A$ with row indices $f_1(i)$ and column indices $f_2(j)$.
We then call the modified procedure \psnealg/2($A^{(k_1,k_2)}$) from the \Cref{appendix:modification-psne} (\Cref{alg:psne-nm}), where we use the query model $\calQ$ (described below) to observe $A^{(k_1,k_2)}_{i,j}$.

After the procedure \psnealg/2$(A^{(k_1,k_2)})$ returns a pair $(\ihat,\:\jhat)$, we compute the set $S:=\{(e_i,e_j):i\in f_1(\ihat),j\in f_2(\jhat)\}$. We return $S$ as the set of basic solutions if the following holds:
\begin{enumerate}
    \item All the entries in $S$ are the PSNE of $A$.
    \item For each $i\notin f_1(\ihat)$, there is an index $j\in f_2(\jhat)$ such that $A_{i,j}<V_A^\star$.
    \item For each $j\notin f_2(\jhat)$, there is an index $i\in f_1(\ihat)$ such that $A_{i,j}>V_A^\star$.
\end{enumerate}
The above conditions can be checked by querying all the entries of $A$ in the set $\{(i,j):i\in f_1(\ihat),j\in[n]\}\cup\{(i,j):i\in [n],j\in f_2(\jhat)\}$. If any one of the conditions above does not hold, we return "failure" instead.

\textbf{Query model $\calQ$ to observe $A^{(k_1,k_2)}_{i,j}$}:
Let $M$ be the submatrix with row indices $f_1(i)$ and column indices $f_2(j)$.
We first query all the entries of $M$ that we have not queried before.
We then compute $\bar M$ and consider it the value of $A^{(k_1,k_2)}_{i,j}$.
% If an entry $(i,j)$ of $A$ was queried earlier, then we directly use the value $A_{i,j}$ observed earlier.

Now, if we want to observe the values in the set $\{A^{(k_1,k_2)}_{i,j}:i\in\calI,j\in \{1,2,\ldots,\binom{n}{k_2}\}\}$, then it suffices to query the entries of $A$ from the set $S_1=\{(i,j):i\in f_{1,\calI}, j\in[n]\}$ where $f_{1,\calI}=\bigcup_{i\in \calI}f_1(i)$.
Since $|f_1(i)|=k_1$, we have that $|S_1|\leq k_1 \cdot n\cdot |\calI|$.
Analogously, if we want to observe the values in the set $\{A^{(k_1,k_2)}_{i,j}:i\in \{1,2,\ldots,\binom{n}{k_1}\},j\in\calJ\}$, then it suffices to query the entries of $A$ from the set $S_2=\{(i,j):i\in [n], j\in f_{2,\calJ}\}$ where $f_{2,\calJ}=\bigcup_{j\in \calJ}f_2(j)$. 
Since $|f_2(j)|=k_2$, we have $|S_2|\leq k_2 \cdot n\cdot|\calJ|$. 

Before start our proof of correctness, we first prove a key proposition

\begin{proposition}\label{prop:multiple-ne}
    Consider the input matrix $A$ with a set $S:=\{(e_i,e_j):e_i\in \calX_\star,e_j\in \calY_\star\}$ of all basic solutions. Let $X:=\{i\in[n]:e_i\in\calX_\star\}$ and $Y:=\{j\in[n]:e_j\in\calY_\star\}$. The following holds true:
    \begin{itemize}
        \item For each $i\notin X$, there is an index $j\in Y$ such that $A_{i,j}<V_A^\star$.
        \item For each $j\notin Y$, there is an index $i\in X$ such that $A_{i,j}>V_A^\star$.
    \end{itemize}
\end{proposition}
\begin{proof}
    First, consider an index $i\notin X$. If $j\in Y$, then we have $A_{i,j}\leq V_A^\star$ as all the basic solutions are PSNE. Now, let $I_y:=\{i\in[n]: V_A^\star=\langle e_i,Ay\rangle\}$. Due to \Cref{technical-multiple-NE}, we have $\bigcap_{y\in \calY_\star}\calI_y=X$. This implies that there is an index $j\in Y$ such that $A_{i,j}<V_A^\star$.

    Similarly, consider an index $j\notin Y$. If $i\in X$, then we have $A_{i,j}\geq V_A^\star$ as all the basic solutions are PSNE. Now, let $I_x:=\{j\in[n]: V_A^\star=\langle x,Ae_j\rangle\}$. Due to \Cref{technical-multiple-NE}, we have $\bigcap_{x\in \calX_\star}\calI_x=Y$. This implies that there is an index $i\in X$ such that $A_{i,j}>V_A^\star$.
\end{proof}


We now prove that the matrix $A^{(k_1,k_2)}$ has a unique PSNE and the inverse mapping of this PSNE corresponds to the set of basic solutions.

\begin{lemma}\label{lem:mul-ne->psne}
Consider the matrix $A^{(k_1,k_2)}$ created using $A$. Let $X:=\{i\in[n]:e_i\in\calX_\star\}$ and $Y:=\{j\in[n]:e_j\in\calY_\star\}$. Then $A^{(k_1,k_2)}$ has a unique PSNE $(\ihat,\jhat)$ such that $\ihat=f_1^{-1}(X)$ and $\jhat=f_2^{-1}(Y)$.
\end{lemma}

\begin{proof}
Recall that $k_1:=|X|$ and $k_2:=|Y|$. Consider the entry $(\ihat,\jhat)$ of $A^{(k_1,k_2)}$ such that  $\ihat=f_1^{-1}(X)$ and $\jhat=f_2^{-1}(Y)$. The sub-matrix $M_0$ of $A$ with row indices $X$ and column indices $Y$ has all the entries equal to $V_A^\star$. Hence $A^{(k_1,k_2)}_{\ihat,\jhat}=V_A^\star$. 

Next consider a $k_1\times k_2$ sub-matrix $M_1$ with row indices $X_1=X$ and column indices $Y_1\neq Y$. Observe that all the entries of $M_1$ have a value at least $V_A^\star$ as all the basic solutions are PSNE. Due to \Cref{prop:multiple-ne}, there exists an entry in $M_1$ with value more than $V_A^\star$. Hence, $A_{\ihat,j}^{(k_1,k_2)}>V_A^\star$ where $j=f_2^{-1}(Y_1)$. Since, $Y_1$ was chosen arbitrarily, we have $A_{\ihat,j}^{(k_1,k_2)}>V_A^\star$ for all $j\neq \jhat$.

Similarly, consider a $k_1\times k_2$ sub-matrix $M_2$ with row indices $X_1\neq X$ and column indices $Y_1=Y$. Observe that all the entries of $M_2$ have a value at most $V_A^\star$ as all the basic solutions are PSNE. Due to \Cref{prop:multiple-ne}, there exists an entry in $M_2$ with value less than $V_A^\star$. Hence, $A_{i,\jhat}^{(k_1,k_2)}<V_A^\star$ where $i=f_1^{-1}(X_1)$. Since, $X_1$ was chosen arbitrarily, we have $A_{i,\jhat}^{(k_1,k_2)}<V_A^\star$ for all $i\neq \ihat$. 

The lemma statement now follows from \Cref{Unique-PSNE}.

\end{proof}

We identify the correct set $S$ of all basic solutions with probability at least $1-\delta$ as the procedure \psnealg/2($A^{(k_1,k_2)}$) returns the unique PSNE $(\ihat,\jhat)$ of $A^{(k_1,k_2)}$ with probability $1-\delta$. Due to \Cref{prop:multiple-ne}, the three conditions towards the end of our randomized procedure is satisfied by $S$ and hence \textsc{Basic} correctly returns set of all basic solutions with probability at least $1-\delta$. Next, we establish the query complexity of \textsc{Basic}$(A,k_1,k_2)$. 

\begin{lemma}
The randomized procedure \textsc{Basic}$(A,k_1,k_2)$ queries $O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of the matrix $A$ where $k:=\max\{k_1,k_2\}$.
\end{lemma}

\begin{proof}First we establish the query complexity of \psnealg/2($A^{(k_1,k_2)}$).
Similar to \psnealg/, at each iteration $t$ of \psnealg/2($A^{(k_1,k_2)}$), we maintained sets $\calX_t$, $\calY_t$, $\Xbar_t$, and $\Ybar_t$ and queried the entries of $A^{(k_1,k_2)}$ in the sets $\{(i,j):i\in\calX_t,j\in \Ybar_t\}$ and $\{(i,j):i\in \Xbar_t,j\in \calY_t\}$.
Using our query model $\calQ$, we can query the entries in these sets by querying at most $2k\cdot n \cdot 2\log(\frac{2n^{2k}}{\delta})\leq 8n\cdot k^2\cdot \log(\frac{2n}{\delta})$ entries from $A$.
This is due to the fact that $\max\{|\Xbar_t|,|\Ybar_t|\}\leq 2\log(\frac{2n^{2k}}{\delta})$. Similar to \psnealg/, we computed indices $\ihat, \jhat$ and queried the entries of $A^{(k_1,k_2)}$ in the sets $\{(\ihat,j):j\in \calY_t\}$ and $\{(i,\jhat):i\in \calX_t\}$.
Again, using our query model $\calQ$, we can query the entries in these sets by querying at most $2kn$ entries from $A$. Now, observe that \psnealg/2($A^{(k_1,k_2)}$) terminates in $t_\star\leq k\cdot \log(n)+1$ iterations.
Hence, \psnealg/2($A^{(k_1,k_2)}$) queries at most $O(nk^3\cdot \log n\cdot\log(\frac{n}{\delta}))$ entries of matrix $A$.

Recall that once we compute a set $S$ of basic solutions using the entry returned by \psnealg/2($A^{(k_1,k_2)}$), we check whether the three conditions towards the end of our randomized procedure is satisfied by $S$ or not. This step requires at most $2kn$ queries. 
\end{proof}

\section{Extra non-unique}
\subsubsection{Algorithm with the knowledge of $k_1,k_2$ and $V_A^\star$.}
Let us first assume that we know the value of the game $V_A^\star$ and the values $k_1:=|\bigcup\limits_{x\in \calX_\star}\supp(x)|$ and $k_2:=|\bigcup\limits_{y\in \calY_\star}\supp(y)|$. Let $A\in\bbR^{n\times n}$ be the input matrix. We construct a matrix $A^{(k_1,k_2,V_A^\star)}\in \bbR^{\binom{n}{k_1} \times \binom{n}{k_2}}$ as follows. First, we create two bijections $f_1:[\binom{n}{k_1}]\rightarrow \binom{[n]}{k_1}$ and $f_2:[\binom{n}{k_2}]\rightarrow \binom{[n]}{k_2}$. Consider indices $i\in [\binom{n}{k_1}]$ and $j\in [\binom{n}{k_2}]$. Let $M$ be the submatrix of $A$ with row indices $f_1(i)$ and column indices $f_2(j)$. Let $\calX_M:=\arg\max_{x\in\simplex_{k_1}}\min_{y\in\simplex_{k_2}}\langle x,My\rangle$ and $\calY_M:=\arg\min_{y\in\simplex_{k_1}}\max_{x\in\simplex_{k_2}}\langle x,My\rangle$. Let $k_{1,M}:=|\bigcup\limits_{x\in \calX_M}\supp(x)|$ and $k_{2,M}:=|\bigcup\limits_{y\in \calY_M}\supp(y)|$. If $V_M^\star\neq V_A^\star$ then we define $A_{i,j}^{(k_1,k_2,V_A^\star)}:=V_M^\star$. If $V_M^\star=V_A^\star$ then we define $A_{i,j}^{(k_1,k_2,V_A^\star)}$ as follows:
\begin{itemize}
    \item If $k_{1,M}=k_1$ and $k_{2,M}=k_2$ then $A_{i,j}^{(k_1,k_2,V_A^\star)}=V_A^\star$
    \item If $k_{1,M}\neq k_1$ and $k_{2,M}\neq k_2$ then $A_{i,j}^{(k_1,k_2,V_A^\star)}=V_A^\star$
    \item If $k_{1,M}= k_1$ and $k_{2,M}\neq k_2$ then $A_{i,j}^{(k_1,k_2,V_A^\star)}=V_A^\star+1$
    \item If $k_{1,M}\neq k_1$ and $k_{2,M}=k_2$ then $A_{i,j}^{(k_1,k_2,V_A^\star)}=V_A^\star-1$
\end{itemize}

Note that there is nothing special about adding and subtracting one. We can replace one with any positive real number. Now we prove the following lemma.
\begin{lemma}\label{lem:high-dim-psne-1}
    Let $i_\star:=f_1^{-1}(\bigcup\limits_{x\in \calX_\star}\supp(x))$ and $j_\star:=f_2^{-1}(\bigcup\limits_{y\in \calY_\star}\supp(y))$. Then $(i_\star,j_\star)$ is the unique PSNE of $A^{(k_1,k_2,V_A^\star)}$.
\end{lemma}
\begin{proof} For the sake of simplicity of presentation, let $\widehat A$ denote the matrix $A^{(k_1,k_2,V_A^\star)}$.
    Now due to \Cref{Unique-PSNE} it suffices to show that 
        $\widehat A_{i,j_\star}<\widehat A_{i_\star,j_\star}<\widehat A_{i_\star,j}$ for all $i\in [\binom{n}{k_1}]\setminus\{i_\star\}$ and $j\in [\binom{n}{k_2}] \setminus\{j_\star\}$.

        Let $(x_\star,y_\star)$ be a Nash equilibrium of $A$ such that the following holds:
        \begin{itemize}
            \item $|\supp(x_\star)|=k_1$ and $|\supp(y_\star)|=k_2$
            \item For all $i\notin \supp(x_\star)$, we have $\langle e_i,Ay_\star\rangle<V_A^\star$
             \item For all $j\notin \supp(y_\star)$, we have $\langle x_\star,Ae_j\rangle>V_A^\star$
        \end{itemize}
         Such an equilibrium exists due to the definition of $k_1,k_2$ and the fact that convex combination of Nash equilibria is also a Nash equilibrium.\textcolor{red}{add a corollary maybe about this last fact}. Let $\widehat x\in \simplex_{k_1}, \widehat y\in\simplex_{k_2}$ be strategies such that for all $i\in f_1(i_\star)$ we have $\widehat x_i=(x_\star)_i$ and for all $j\in f_2(j_\star)$ we have $\widehat y_j=(y_\star)_j$. 

        First we claim that $\widehat A_{i_\star,j_\star}=V_A^\star$. Consider the submatrix $M$ of $A$ with row indices $f_1(i_\star)$ and column indices $f_2(j_\star)$. As $|\supp(x_\star)|=k_1$ and $|\supp(y_\star)|=k_2$, we have $\langle x,M \widehat y\rangle=V_A^\star$ for all $x\in \simplex_{k_1}$ and $\langle \widehat x,M y\rangle=V_A^\star$ for all $y\in \simplex_{k_2}$. Hence $(\widehat x,\widehat y)$ is the Nash equilibrium of $M$ which implies that $V_M^\star=\langle \widehat x,M\widehat y\rangle=V_A^\star$. As $|\supp(\widehat x)|=k_1$ and $|\supp(\widehat y)|=k_2$ we have $\widehat A_{i_\star,j_\star}=V_A^\star$.

        Next consider an index $i\in [\binom{n}{k_1}]$ such that $f_1(i)\cap f_1(i_\star)=\emptyset$. Now we claim that $\widehat A_{i,j_\star}<V_A^\star$.  Consider the submatrix $M$ of $A$ with row indices $f_1(i)$ and column indices $f_2(j_\star)$. Now we have the following:
\[
V_{M}^\star=\min_{y\in\simplex_{k_2}}\max_{i\in f_1(i)}\langle e_i,My\rangle\leq \max_{i\in f_1(i)}\langle e_i,M \widehat y\rangle<V_A^\star.
\]
The last inequality follows from our choice of $(x_\star,y_\star)$ above and $f_1(i)\cap f_1(i_\star)=\emptyset$. Similarly we can show that for any $j\in [\binom{n}{k_2}]$ such that $f_2(j)\cap f_2(j_\star)=\emptyset$, we have $\widehat A_{i_\star,j}>V_A^\star$.

Next consider an index $i\in [\binom{n}{k_1}]\setminus\{i_\star\}$ such that $f_1(i)\cap f_1(i_\star)\neq\emptyset$. Now we claim that $\widehat A_{i,j_\star}<V_A^\star$.  Consider the submatrix $M$ of $A$ with row indices $f_1(i)$ and column indices $f_2(j_\star)$. Now we have the following:
\[
V_{M}^\star=\min_{y\in\simplex_{k_2}}\max_{i\in f_1(i)}\langle e_i,My\rangle\leq \max_{i\in f_1(i)}\langle e_i,M \widehat y\rangle= V_A^\star.
\]
Recall the definition of $\calX_M, \calY_M, k_{1,M}$ and $k_{2,M}$. If $V_M^\star<V_A^\star$ then we have $\widehat A_{i,j_\star}<V_A^\star$. Let us consider the case when $V_M^\star=V_A^\star$. In this case, we have $\widehat y\in \calY_{M}$ which implies that $k_{2,M}=k_2$. Consider $x\in \calX_{M}$. For any $i\notin f_1(i)\cap f_1(i_\star)$ we have $\langle e_i,M\widehat y\rangle<V_A^\star$. This implies that $\supp(x)\subseteq f_1(i)\cap f_1(i_\star)$. As $x$ was chosen arbitrarily, we have $\bigcup\limits_{x\in \calX_\star}\supp(x)\subseteq f_1(i)\cap f_1(i_\star)$. As $f_1(i)\neq f_1(i_\star)$ this implies $|f_1(i)\cap f_1(i_\star)|<k_1$. This implies that $k_{1,M}\neq k_1$. Hence due to our construction, we have $\widehat A_{i,j_\star}=V_A^\star-1<V_A^\star$. Similarly we can show that for any $j\in [\binom{n}{k_2}]\setminus\{j_\star\}$ such that $f_2(j)\cap f_2(j_\star)\neq\emptyset$, we have $\widehat A_{i_\star,j}>V_A^\star$.

Combining all the cases above, we have  $\widehat A_{i,j_\star}<\widehat A_{i_\star,j_\star}<\widehat A_{i_\star,j}$ for all $i\in [\binom{n}{k_1}]\setminus\{i_\star\}$ and $j\in [\binom{n}{k_2}] \setminus\{j_\star\}$.


\end{proof}

\textbf{Query oracle $\calQ$ to observe row $\hat i$ and column $\hat j$ of $A^{(k_1,k_2,V_A^\star)}$}:
Recall that $A^{(k_1,k_2)}_{i,j}$ only depends on the entries in the submatrix $M$ with row indices $f_1(i)$ and column indices $f_2(j)$.
Hence, if we want to observe the values in the set $\{A^{(k_1,k_2,V_A^\star)}_{\hat i,j}:j\in \{1,2,\ldots,\binom{n}{k_2}\}\}$, then it suffices to query the entries of $A$ from the set $S_1=\{(i,j):i\in f_{1}(\hat i), j\in[n]\}$.
Since $|f_1(\hat i)|=k_1$, we have that $|S_1|= k_1 \cdot n$.
Analogously, if we want to observe the values in the set $\{A^{(k_1,k_2)}_{i,\hat j}:i\in \{1,2,\ldots,\binom{n}{k_1}\}\}$, then it suffices to query the entries of $A$ from the set $S_2=\{(i,j):i\in [n], j\in f_{2}(\hat j)\}$. 
Since $|f_2(j)|=k_2$, we have $|S_2|= k_2 \cdot n$. 


Now we describe $\textsc{Nash}$, a randomized algorithm that finds $\calX_\star$ and $\calY_\star$ when provided with the values $k_1,k_2$ and $V_A^\star$. 

\textbf{Description of the randomized procedure } \textsc{Nash}$(A,\delta,k_1,k_2,V_A^\star)$:
Let $A\in\bbR^{n\times n}$ be the input matrix. Recall the construction of the matrix $A^{(k_1,k_2,V_A^\star)}\in \bbR^{\binom{n}{k_1} \times \binom{n}{k_2}}$ from above. We now call the procedure \psnealg/($A^{(k_1,k_2,V_A^\star)},\delta$), where we use the query oracle $\calQ$ to observe $A^{(k_1,k_2,V_A^\star)}_{i,j}$.

Let $(\hat i, \hat j)$ be the pair returned by the procedure \psnealg/$(A^{(k_1,k_2,V_A^\star)},\delta)$. Let $M_1$ be the submatrix of $A$ with row indices $f_1(\hat i)$ and column indices $[n]$, and $M_2$ be the submatrix of $A$ with row indices $[n]$ and column indices $f_2(\hat j)$. Let $\calX_{M_1}:=\arg\max_{x\in\simplex_{k_1}}\min_{y\in\simplex_{n}}\langle x,M_1y\rangle$ and $\calY_{ M_2}:=\arg\min_{y\in\simplex_{k_2}}\max_{x\in\simplex_{n}}\langle x,M_2y\rangle$. For any vector $v$ and the set of indices $\calS=\{i_1,\ldots, i_{\ell}\}$, let $v_\calS$ denote the vector $(v_{i_1},\ldots,v_{i_{\ell}})$. Let $\calX_A:=\{x\in\simplex_n:x_{f_1(\hat i)}\in \calX_{M_1} \}$ and $\calY_A:=\{y\in\simplex_m:y_{f_2(\hat j)}\in \calY_{M_2} \}$. We return $\calX_A\times \calY_A$ as the set of Nash equilibria if the following conditions hold:
\begin{enumerate}
    \item[(C1)] $V_{M_1}^\star=V_A^\star$ and $\bigcap\limits_{x\in\calX_A}I_x=f_2(\hat j)$ where $I_x=\{j\in[n]: V_A^\star=\langle x, A e_j\rangle\}$. 
    \item[(C2)] $V_{M_2}^\star=V_A^\star$ and $\bigcap\limits_{y\in\calY_A}I_y=f_1(\hat i)$ where $I_y=\{i\in[n]: V_A^\star=\langle e_i, A y\rangle\}$.
\end{enumerate}

\textcolor{red}{Ensure that these conditions are indeed correct.}

The above conditions can be checked by querying all the entries of $A$ in the set $\{(i,j):i\in f_1(\hat i),j\in[n]\}\cup\{(i,j):i\in [n],j\in f_2(\hat j)\}$. If any one of the conditions above does not hold, we return "failure" instead.

Now we state the guarantees of our randomized procedure.
\begin{lemma}\label{lem:alg-multiple-ne}
Consider a matrix game $A\in\bbR^{n\times n}$. Now we have the following:
\begin{itemize}
    \item The procedure \textsc{Nash}$(A,\delta,k_1,k_2,V_A^\star)$ queries at most $O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of $A$. 
    \item With probability at least $1-\delta$, the procedure \textsc{Nash}$(A,\delta,k_1,k_2,V_A^\star)$ returns $\calX_\star\times \calY_\star$. 
\end{itemize}

\end{lemma}
\begin{proof}
Due to \Cref{lem:psne-query}, the number of calls made to the query oracle $\calQ$ is at most $O(\log(n^k)\cdot\log(\frac{n^k}{\delta}))\leq O(k^2\cdot \log(n)\cdot\log(\frac{n}{\delta}))$. Each call to the query oracle $\calQ$ takes $O(nk)$ queries from the input matrix $A$. Moreover, to check the conditions $(C1)$ and $(C2)$ it takes $O(nk)$ queries. Hence, the procedure \textsc{Nash}$(A,\delta,k_1,k_2,V_A^\star)$ queries at most $O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of $A$.   

Recall the construction of the sets $\calX_A$ and $\calY_A$. Due to \Cref{lem:high-dim-psne-1} and \Cref{lem:psne-correct}, the procedure \psnealg/$(A^{(k_1,k_2,V_A^\star)},\delta)$ returns the pair $(\istar, \jstar)$ with probability at least $1-\delta$, where $i_\star:=f_1^{-1}(\bigcup\limits_{x\in \calX_\star}\supp(x))$ and $j_\star:=f_2^{-1}(\bigcup\limits_{y\in \calY_\star}\supp(y))$. This implies that with probability at least $1-\delta$, the sets $\calX_A=\calX_\star$ and $\calY_A=\calY_\star$. As the set $\calX_\star\times\calY_\star$ satisfies the conditions (C1) and (C2), with probability at least $1-\delta$, the procedure \textsc{Nash}$(A,\delta,k_1,k_2,V_A^\star)$ returns $\calX_\star\times \calY_\star$. 
\end{proof}
\subsubsection{Relaxing the assumption on the knowledge of $V_A^\star$}
Let us now assume that we know only the values $k_1:=|\bigcup\limits_{x\in \calX_\star}\supp(x)|$ and $k_2:=|\bigcup\limits_{y\in \calY_\star}\supp(y)|$. Let $A\in\bbR^{n\times n}$ be the input matrix. We construct a matrix $A^{(k_1,k_2)}\in \bbR^{\binom{n}{k_1} \times \binom{n}{k_2}}$ as follows. First, we create two bijections $f_1:[\binom{n}{k_1}]\rightarrow \binom{[n]}{k_1}$ and $f_2:[\binom{n}{k_2}]\rightarrow \binom{[n]}{k_2}$. Consider indices $i\in [\binom{n}{k_1}]$ and $j\in [\binom{n}{k_2}]$. Let $M$ be the submatrix of $A$ with row indices $f_1(i)$ and column indices $f_2(j)$. We now define $A_{i,j}^{(k_1,k_2)}:=V_M^\star$.

Now we prove the following lemma.
\begin{lemma}
    Let $i_\star:=f_1^{-1}(\bigcup\limits_{x\in \calX_\star}\supp(x))$ and $j_\star:=f_2^{-1}(\bigcup\limits_{y\in \calY_\star}\supp(y))$. Then $(i_\star,j_\star)$ is a PSNE of $A^{(k_1,k_2)}$ and $A^{(k_1,k_2)}_{\istar,\jstar}=V_A^\star$.
\end{lemma}
\begin{proof}
\textcolor{red}{Fix the notational abuse of $\simplex_{k_1}$ later on and make it short perhaps. We can push this to appendix.}

For the sake of simplicity of presentation, let $\widehat A$ denote the matrix $A^{(k_1,k_2)}$. Let $(x_\star,y_\star)$ be a Nash equilibrium of $A$ such that the following holds:
        \begin{itemize}
            \item $|\supp(x_\star)|=k_1$ and $|\supp(y_\star)|=k_2$
            \item For all $i\notin \supp(x_\star)$, we have $\langle e_i,Ay_\star\rangle<V_A^\star$
             \item For all $j\notin \supp(y_\star)$, we have $\langle x_\star,Ae_j\rangle>V_A^\star$
        \end{itemize}
         Such an equilibrium exists due to the definition of $k_1,k_2$ and the fact that convex combination of Nash equilibria is also a Nash equilibrium. Let $\widehat x\in \simplex_{k_1}, \widehat y\in\simplex_{k_2}$ be strategies such that for all $i\in f_1(i_\star)$ we have $\widehat x_i=(x_\star)_i$ and for all $j\in f_2(j_\star)$ we have $\widehat y_j=(y_\star)_j$. 

        First we claim that $\widehat A_{i_\star,j_\star}=V_A^\star$. Consider the submatrix $M$ of $A$ with row indices $f_1(i_\star)$ and column indices $f_2(j_\star)$. As $|\supp(x_\star)|=k_1$ and $|\supp(y_\star)|=k_2$, we have $\langle x,M \widehat y\rangle=V_A^\star$ for all $x\in \simplex_{k_1}$ and $\langle \widehat x,M y\rangle=V_A^\star$ for all $y\in \simplex_{k_2}$. Hence $(\widehat x,\widehat y)$ is the Nash equilibrium of $M$ which implies that $V_M^\star=\langle \widehat x,M\widehat y\rangle=V_A^\star$. As $|\supp(\widehat x)|=k_1$ and $|\supp(\widehat y)|=k_2$ we have $\widehat A_{i_\star,j_\star}=V_A^\star$.

        Next consider an index $i\in [\binom{n}{k_1}]$. Now we claim that $\widehat A_{i,j_\star}\leq V_A^\star$.  Consider the submatrix $M$ of $A$ with row indices $f_1(i)$ and column indices $f_2(j_\star)$. Now we have the following:
\[
V_{M}^\star=\min_{y\in\simplex_{k_2}}\max_{i\in f_1(i)}\langle e_i,My\rangle\leq \max_{i\in f_1(i)}\langle e_i,M \widehat y\rangle\leq V_A^\star.
\]
The last inequality follows from our choice of $(x_\star,y_\star)$ above. Similarly we can show that for any $j\in [\binom{n}{k_2}]$, we have $\widehat A_{i_\star,j}\geq V_A^\star$.
\end{proof}

\textbf{Query oracle $\calQ$ to observe row $\hat i$ and column $\hat j$ of $A^{(k_1,k_2)}$}:
Recall that $A^{(k_1,k_2)}_{i,j}$ only depends on the entries in the submatrix $M$ with row indices $f_1(i)$ and column indices $f_2(j)$.
Hence, if we want to observe the values in the set $\{A^{(k_1,k_2,V_A^\star)}_{\hat i,j}:j\in \{1,2,\ldots,\binom{n}{k_2}\}\}$, then it suffices to query the entries of $A$ from the set $S_1=\{(i,j):i\in f_{1}(\hat i), j\in[n]\}$.
Since $|f_1(\hat i)|=k_1$, we have that $|S_1|= k_1 \cdot n$.
Analogously, if we want to observe the values in the set $\{A^{(k_1,k_2)}_{i,\hat j}:i\in \{1,2,\ldots,\binom{n}{k_1}\}\}$, then it suffices to query the entries of $A$ from the set $S_2=\{(i,j):i\in [n], j\in f_{2}(\hat j)\}$. 
Since $|f_2(j)|=k_2$, we have $|S_2|= k_2 \cdot n$.


Now we describe $\textsc{AlgoNE}$, a randomized algorithm that finds $\calX_\star$ and $\calY_\star$ when provided with the values $k_1$ and $k_2$.  

\textbf{Description of the randomized procedure } \textsc{AlgoNE}$(A,\delta,k_1,k_2)$:
Let $A\in\bbR^{n\times n}$ be the input matrix. Recall the construction of the matrix $A^{(k_1,k_2)}\in \bbR^{\binom{n}{k_1} \times \binom{n}{k_2}}$ from above. We now call the procedure \psnealg/($A^{(k_1,k_2)},\frac{\delta}{2}$), where we use the query oracle $\calQ$ to observe $A^{(k_1,k_2)}_{i,j}$. Let $\calV$ be the set of values returned by \psnealg/($A^{(k_1,k_2)},\frac{\delta}{2}$). For each $V\in \calV$, we call the procedure \textsc{Nash}($k_1,k_2,V$). If there is a $V\in \calV$ such that \textsc{Nash}($A,\frac{\delta}{2},k_1,k_2,V$) returns a set of Nash equilibria $\calX_A\times \calY_A$, we return this set as the set of Nash equilibria. If there is more than one such $V$, choose one of them arbitrarily and return the set $\calX_A\times \calY_A$. If for all  $V\in \calV$, \textsc{Nash}($A,\frac{\delta}{2},k_1,k_2,V$) returns a "failure", then we return "failure".

\begin{lemma}
Consider a matrix game $A\in\bbR^{n\times n}$. Now we have the following:
\begin{itemize}
    \item The procedure \textsc{AlgoNE}$(A,\delta,k_1,k_2)$ queries at most $O(nk^4\cdot \log^2 n\cdot \log(\frac{n}{\delta}))$ entries of $A$. 
    \item With probability at least $1-\delta$, the procedure \textsc{AlgoNE}$(A,\delta,k_1,k_2)$ returns $\calX_\star\times \calY_\star$. 
\end{itemize}
\end{lemma}
\begin{proof}
    Due to \Cref{lem:psne-query}, the number of calls made by \psnealg/($A^{(k_1,k_2)},\frac{\delta}{2}$) to the query oracle $\calQ$ is at most $O(\log(n^k)\cdot\log(\frac{n^k}{\delta}))\leq O(k^2\cdot \log(n)\cdot\log(\frac{n}{\delta}))$. Each call to the query oracle $\calQ$ takes $O(nk)$ queries from the input matrix $A$. Hence, the procedure \psnealg/($A^{(k_1,k_2)},\frac{\delta}{2}$) queries at most $O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of $A$. Next, recall that due to \Cref{lem:alg-multiple-ne}, each call to the procedure \textsc{Nash}($A,\frac{\delta}{2},k_1,k_2,V$) queries at most $O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of $A$. Due to \Cref{lem:non-unique-psne}, $|\calV|\leq 2k\log(n)+1$. Hence, the procedure \textsc{AlgoNE}$(A,\delta,k_1,k_2)$ queries at most $O(nk^4\cdot \log^2 n\cdot \log(\frac{n}{\delta}))$ entries of $A$.  
    
     If there is a $V\in \calV$ such that \textsc{Nash}($A,\frac{\delta}{2},k_1,k_2,V$) returns a set $\calX_A\times \calY_A$ then $\calX_A\times\calY_A=\calX_\star\times\calY_\star$ as $\calX_\star\times\calY_\star$ is the only set that satisfies the conditions (C1) and (C2). Due to \Cref{lem:non-unique-psne}, with probability at least $1-\frac{\delta}{2}$, $\calV_A^\star\in\calV$. Due to \Cref{lem:alg-multiple-ne}, with probability at least $1-\frac{\delta}{2}$, \textsc{Nash}($A,\frac{\delta}{2},k_1,k_2,V_A^\star$) returns the set $\calX_\star\times \calY_\star$. Due to union bound, with probability at least $1-\delta$, the procedure 

     \noindent
     \textsc{AlgoNE}$(A,\delta,k_1,k_2)$ returns $\calX_\star\times \calY_\star$.  
\end{proof}

\textcolor{red}{Merge both the sections into one single algorithm.}


==> lower_bound.tex <==
\section{A Lower Bound for Finding the Nash Equilibrium}\label{sec:lower}
%\arnab{I will make the changes suggested by Kevin and Lily sometime today.}
%\arnab{I am open to pushing this section back and showing the algorithms first.}
It is straightforward to show that changing the entries in the submatrix $M$ with row indices $[n]$ and column indices $\supp(\ystar)$ can change the Nash equilibrium of the input matrix $A\in\bbR^{n\times n}$.
This raises the following question: \emph{Is it necessary to query a constant fraction of entries in $M$ in order to compute the Nash equilibrium of $A$?}
The following theorem answers this question in the affirmative.

\begin{theorem}\label{thm:lower-bound:new}
Let $\calA$ be any randomized algorithm that correctly computes the Nash equilibrium of the input matrix.
Let $\tau(M)$ denote the number of entries queried from the matrix $M$ by $\calA$.
Then, there exists an input matrix $A\in \bbR^{n\times n}$ with a unique Nash equilibrium $(\xstar,\ystar)$ such that $\bbE[\tau(A)]\geq \frac{nk}{8}$ where $k=|\supp(\ystar)|$ and the randomness in $\tau(A)$ is due to $\calA$ only.
\end{theorem}

%\kevin{This theorem statement is confusing. Is $X$ distinct from the input matrix? Why not state as $\inf_A max_X$?}
%\arnab{The theorem aims to lower bound the expected query complexity of the algorithm. So it tries to say that for any randomized algorithm there will be an input matrix for which the expected query complexity is high. Formally, I meant to show the following $\max_A\bbE_{\alg\sim\calA}[\tau(\alg,A)]\geq nk/8$ precisely. }
%\kevin{Not clear if big-O is referring to $n$ or $k$, or both}
%\arnab{It is referring to both. big-O and big-Omega is only hiding the constants.}

\begin{proof}
The proof proceeds by considering two cases: (1) $k\leq \frac{n}{2}$ and (2) $k>\frac{n}{2}$. 
We prove case 1 here, and defer the proof of case 2 to Appendix \ref{appendix:lower}.

Suppose that $k\leq \frac{n}{2}$.
Consider $\ihat\in[n]\setminus[k]$ and $\jhat\in[k]$.
Let $A^{(\ihat,\jhat)}\in \bbR^{n\times n}$ denote a matrix such that the following holds: i) entry $(\ihat,\jhat)$ %of $A^{(\ihat,\jhat)}$ 
has a value of two, ii) all entries $(i,j)$ 
%of $A^{(\ihat,\jhat)}$ 
have a value three for $i\in [n]$ and $j\in[n]\setminus [k]$, iii) the entries $(i,i)$ %of $A^{(\ihat,\jhat)}$ 
have a value one for all $i\in [k]$, and iv) rest of the entries $(i,j)$ have a value zero.


Now, observe that from the perspective of the column player, columns $1,2,\ldots,k$ strictly dominate the columns $k+1,k+2,\ldots,n$.
Hence, the zero-sum game effectively reduces to the sub-matrix $B_1$ with row indices $[n]$ and column indices $[k]$.
Now, observe that from the perspective of the row player, row $\ihat$ strictly dominates the rows with indices $\{k+1,\ldots,n\}\cup\{\jhat\}\setminus\{\ihat\}$ in the sub-matrix $B_1$.
Hence, the zero-sum game effectively reduces to the sub-matrix $B_2$ with row indices $[k]\cup\{\ihat\}\setminus\{\jhat\}$ and column indices $[k]$.
This $k\times k$ sub-matrix is equivalent (up to a row permutation) to a diagonal matrix  with all diagonal entries having value one except one entry which has value two.
Hence, it is easy to observe that this matrix has a unique Nash equilibrium $(\xhat,\yhat)$ such that $\xhat_i=\frac{1}{k-1/2}$ for all $i\in [k]\setminus\{\jhat\}$ and $\xhat_{\ihat}=\frac{1/2}{k-1/2}$ and, analogously,  $\yhat_j=\frac{1}{k-1/2}$ for all $j\in [k]\setminus\{\jhat\}$ and $\yhat_{\jhat}=\frac{1/2}{k-1/2}$.
% be the matrix that satisfies
% \begin{align*}
%     A_{i,j}^{(\ihat,\jhat)} = 
%     \begin{cases}
%     2,& (i,\:j) = (\ihat,\:\jhat)\\
%     3,& i\in [n],\: j\in[n]\setminus [k] \\
%     1,& i=j\in [k]\\
%     0,& \text{otherwise}.
%     \end{cases}
% \end{align*}


% From the perspective of the column (min) player, columns in $[k]$ are never a best response and can be eliminated. For the row (max) player, $\ihat$ strictly dominates the other rows in $[n]\setminus [k]$ as well as $\jhat$, given that the column player will choose a column in $[k]$.

% Hence, this game effectively reduces to the game defined by the submatrix $B_1$ with row indices $[n]$ and column indices $[k]$.
% Now, observe that from the perspective of a row player, row $\ihat$ strictly dominates the rows with indices $\{k+1,\ldots,n\}\cup\{\jhat\}\setminus\{\ihat\}$ in the sub-matrix $B_1$.
% Hence, the game further reduces to the sub-matrix $B_2$ with row indices $[k]\cup\{\ihat\}\setminus\{\jhat\}$ and column indices $[k]$.
% After eliminating these non-viable strategies, the resulting submatrix is equivalent to an $\frac{n}{2}\times \frac{n}{2}$ diagonal matrix with all diagonal being equal to $1$ except one entry which is equal to $2$.
% This submatrix shows that $A$ has a unique Nash equilibrium 
% $(\xstar,\ystar)$ with $(\xstar)_i=\frac{1}{k-1/2}$ for all $i\in [k]\setminus\{\jhat\}$ and $(\xstar)_{\ihat}=\frac{1/2}{k-1/2}$; and similarly, with $(\ystar)_j=\frac{1}{k-1/2}$ for all $j\in [k]\setminus\{\jhat\}$ and $(\ystar)_{\jhat}=\frac{1/2}{k-1/2}$.  

Now, consider the set of input instances $\calM:=\{A^{(i,j)}:i\in[n]\setminus[k],j\in[k]\}$.
Observe that no two instances of $\calM$ have the same Nash equilibrium. Let us assume that the randomized algorithm $\calA$ is a distribution over a set $\calD$ of deterministic algorithms.
Fix a deterministic instance $\alg\in \calD$. We now claim that there is a subset $\calM_1\subseteq \calM$ of size at least $\frac{|\calM|}{2}$ such that $\alg$ queries at least $\frac{nk}{4}$ entries from each input instance in $\calM_1$.
%\kevin{Very confusing to have $A$ represent both a matrix in the rest of the text, and here $A$ represent an algorithm. Perhaps use {\sf Alg} instead?} \ljr{Agreed.}
%\arnab{Thanks for making the changes. I will make changes to the notation in other parts of the proof too today.}
As $\alg$ computes the correct Nash equilibrium of the input matrix, by construction there exists a matrix $M\in\calM$ such that the first $\frac{nk}{4}$ entries of $M$ queried by $\alg$ have values in $\{0,1,3\}$. 
% \kevin{I don't understand this last sentence. Why does it need to take $nk/4$ queries from the input matrix before stopping? Its a needle in a haystack of size $(n-k)k$ so it makes sense. But I don't see why the algoithm must take $nk/4$ queries, this seems like what you're trying to prove in the first place  }\ljr{I am also confused by this...}\arnab{Will clarify this part today.}
Denoting this set of entries as $S$, $\alg$ will query all the entries in $S$ from each of the input matrices in {$\calM_1=\{A^{(i,j)}\mid(i,j)\notin S,\ i\in[n]\setminus[k],\ j\in[k]\}$}, as each $A\in\calM_1$ is equal to $M$ on $S$ and every matrix in $\calM_1$ has a different Nash equilibrium.
Let $\tau(\alg,A)$ denote the number of queries taken by $\alg$ from an input matrix $A$.
As $|\calM_1|\geq |\calM|-\frac{nk}{4}\geq \frac{|\calM|}{2}$, we have $\bbE_{A\sim\text{Unif}(\calM)}[\tau(\alg,A)]\geq \frac{1}{2}\cdot \frac{nk}{4}=\frac{nk}{8}$. Due to Yao's lemma, we have that
\[
\max_{A\in\calM}\E[\tau(A)] \geq \min_{\alg\in\calD}\E_{A\sim\text{Unif}(\calM)}[\tau(\alg,A)] \geq \frac{nk}{8}.
\] 
% \kevin{Why are we using Yao's lemma here? Can't we just end with $\inf_{A \in \calA} \max_{X \in \calM} \tau(A,X) \geq \inf_{A \in \calA} \bbE_{X\sim\text{Unif}(\calM)}[\tau(A,X)]\geq \frac{1}{2}\cdot \frac{nk}{4}=\frac{nk}{8}$}
% \arnab{I meant to show the following $\max_A\bbE_{\alg\sim\calA}[\tau(\alg,A)]\geq nk/8$ precisely. Hence I used Yao's lemma. The expression $\inf_{A \in \calA} \max_{X \in \calM} \tau(A,X)$ doesn't say anything about the expected query complexity of an algorithm.}
% \ljr{Agreed. this is a little unclear. its also strange to have $\alg\sim \calA$ and $\alg\in \calA$ since that is overloading the notion of $\calA$.}
% \arnab{This is what Ross and I meant: Any randomized algorithm $\calA$ is essentially a distribution over a set of deterministic algorithms. So $\alg\sim \calA$ means one initialization of the random algo and $\alg\in \calA$ is essentially chosing one deterministic algo from set of determinisitc algorithms. }
%\ljr{That is fine but that is still overloading the notation since $\mathcal{A}$ is not set or a space but distribution so it doesnt make sense to say $\alg\in \mathcal{A}$ in that sense. You could say $\alg\in supp(\mathcal{A})$ that would be more accurate.}
%Similarly, we prove the other case $k>\frac{n}{2}$ in the Appendix \ref{appendix:lower}.
\end{proof}


==> randomized_ne_alg.tex <==
\subsection{A Randomized Algorithm to Find the Unique Nash Equilibrium }\label{section:random:msne}
% \arnab{This section is a bit notation heavy, especially notations like $\simplex_\calI$. Any simplification of this section would be helpful.}
% \ross{you might want to give the PSNE alg a different name (doesn't have to be cute), just so we're not overloading, bc we use "PSNE" a lot. }
% \ljr{I personally do not like acronyms like this in the first place and would prefer if we spell it out. But I would prefer an acronym over some made up name. Definitely dont like that we do PSNE as a name and as an operator---i.e., PSNE$(A)$ and PSNE="pure strategy Nash equilibrium"}
% \ross{I think something descriptive would be better than just PSNE -- even \textsc{FindPSNE} or something like that would be better just to make a distinction. In any case, I made it a macro (\textbackslash psnealg/, note the trailing slash) in macros.sty, so make any change there}
%\noindent

\textcolor{red}{Decide if you want this section or not. Has some nice value to it but consumes space as well.}

In this section, we give a support enumeration-based randomized procedure that achieves the following result.
Throughout, let $\simplex_{\calI}$ denote the probability simplex over the set of indices $\calI$.

\begin{theorem}\label{thm:mixed}
Consider a matrix game $A\in\bbR^{n\times n}$ that has a unique Nash equilibrium $(\xstar,\ystar)$.
Let $k:=|\supp(\xstar)|$.
There is a randomized procedure that with probability at least $1-\delta$ queries at most $O(nk^4\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of $A$ and computes $(\xstar,\ystar)$. 
\end{theorem}

Let us assume that we know the value of $k=|\supp(\xstar)|$. Towards the end of this section, we relax this assumption. 

\textbf{Description of the algorithm:}
Let $A\in\bbR^{n\times n}$ be the input matrix.
We construct a matrix $A^{(k)}\in \bbR^{\binom{n}{k} \times \binom{n}{k}}$ as follows.
First, we create a bijection $f:\binom{n}{k}\rightarrow \binom{[n]}{k}$.
Let $A^{(k)}_{i,j}=V_C^\star$ where $C$ is the sub-matrix of $A$ with row indices $f(i)$ and column indices $f(j)$.
We then call the procedure \psnealg/($A^{(k)}$) from the previous section (\Cref{alg:psne}), where we use the query model $\calQ$ (described below) to observe $A^{(k)}_{i,j}$.

After the procedure \psnealg/$(A^{(k)})$ returns a pair $(\ihat,\:\jhat)$, we compute the following:
\begin{equation*}
    \xhat=\arg\max_{x\in \simplex_{f(\ihat)}}\min_{y\in\simplex_{f(\jhat)}}\langle x, \Ahat y\rangle,\quad \yhat=\arg\min_{y\in \simplex_{f(\jhat)}}\max_{x\in\simplex_{f(\ihat)}}\langle x, \Ahat y\rangle
\end{equation*}
where $\Ahat$ is the sub-matrix of $A$ with row indices $f(\ihat)$ and column indices $f(\jhat)$.
We then return the pair $(\xstar,\ystar)\in\simplex_n\times\simplex_n$ as the Nash equilibrium of $A$ where $(\xstar)_i=\xhat_i$ for all $i\in f(\ihat)$ and $(\ystar)_j=\yhat_j$ for all $j\in f(\jhat)$.

\textbf{Query model $\calQ$ to observe $A^{(k)}_{i,j}$}:
Let $C$ be the submatrix with row indices $f(i)$ and column indices $f(j)$.
We first query all the entries of $C$ that we have not queried before.
We then compute $V_C^\star$ and consider it the value of $A^{(k)}_{i,j}$.
% If an entry $(i,j)$ of $A$ was queried earlier, then we directly use the value $A_{i,j}$ observed earlier.

Now, if we want to observe the values in the set $\{A^{(k)}_{i,j}:i\in\calX,j\in \{1,2,\ldots,\binom{n}{k}\}\}$, then it suffices to query the entries of $A$ from the set $S_1=\{(i,j):i\in f_\calX, j\in[n]\}$ where $f_\calX=\bigcup_{i\in \calX}f(i)$.
Since $|f(i)|=k$, we have that $|S_1|\leq k \cdot n\cdot |\calX|$.
Analogously, if we want to observe the values in the set $\{A^{(k)}_{i,j}:i\in \{1,2,\ldots,\binom{n}{k}\},j\in\calY\}$, then it suffices to query the entries of $A$ from the set $S_2=\{(i,j):i\in [n], j\in f_\calY\}$ where $f_\calY=\bigcup_{j\in \calY}f(j)$. 
Since $|f(j)|=k$, we have $|S_2|\leq k \cdot n\cdot|\calY|$.

We now prove the following lemma that is helpful to show that the matrix $A^{(k)}$ has a unique PSNE.

\begin{lemma}\label{lem:ne->psne:1}
Consider a matrix $M\in \bbR^{n\times k}$.
Let $M$ have a unique Nash equilibrium $(\xstar,\ystar)$ such that $|\supp(\xstar)|=k$.
Consider a $k\times k$ submatrix $M_1$ of $M$ with row indices $\calI$.
If $\calI\neq \supp(\xstar)$ then $V_{M_1}^\star<V_M^\star$. 
\end{lemma}

\begin{proof}
First, recall that $V_M^\star>\max_{i\notin \supp(\xstar)}\langle e_i,M\ystar\rangle$ and $V_M^\star=\langle e_i,M\ystar\rangle$ for any $i\in \supp(\xstar)$.
We now divide our analysis into two cases. 

\textbf{Case 1}: $\calI\cap \supp(\xstar)=\emptyset$.
In this case, we have that
\[
V_{M_1}^\star=\min_{y\in\simplex_k}\max_{i\in\calI}\langle e_i,M_1y\rangle\leq \max_{i\in\calI}\langle e_i,M_1\ystar\rangle<V_M^\star.
\]

\textbf{Case 2}: $\calI\cap \supp(\xstar)\neq\emptyset$.
In this case, we have that 
\[
V_{M_1}^\star=\min_{y\in\simplex_k}\max_{i\in\calI}\langle e_i,M_1y\rangle\leq \max_{i\in\calI}\langle e_i,M_1\ystar\rangle= V_M^\star.
\]
Let us assume that $V_M^\star=V_{M_1}^\star$.
Then, we have that $V_{M_1}^\star=\max_{i\in\calI}\langle e_i,M_1\ystar\rangle$.
This implies $\ystar\in \argmin_{y\in \simplex_k}\max_{i\in\calI}\langle e_i,M_1y\rangle$. 

Now, consider $x^{(1)}\in\argmax_{x\in\simplex_{\calI} }\min_{y\in \simplex_k}\langle x,M_1y\rangle$.
Observe that $(x^{(1)},\ystar)$ is a Nash equilibrium of $M_1$.
Hence, we have 
\[
\langle x^{(1)},M_1\ystar\rangle=V_{M_1}^\star=V_{M}^\star=\max_{x\in\simplex_n}\langle x,M\ystar\rangle\quad\text{and}\quad \langle x^{(1)},M_1\ystar\rangle=\min_{y\in\simplex_k}\langle x^{(1)}, M_1y\rangle.
\]

Let $x^{(2)}\in \simplex_n$ where $x^{(2)}_i=x^{(1)}_i$ for all $i\in \calI$. Since $\supp(x^{(2)})\subseteq\calI$, we have that $\langle x^{(2)},M\ystar\rangle=\langle x^{(1)},M_1\ystar\rangle$.
We can then deduce that \[\langle x^{(2)},M\ystar\rangle= \max_{x\in\simplex_n}\langle x,M\ystar\rangle\quad\text{and}\quad\langle x^{(2)},M\ystar\rangle= \min_{y\in\simplex_k}\langle x^{(2)}, My\rangle,\] so that $(x^{(2)},\ystar)$ is a Nash equilibrium of $M$.
However $\supp(x^{(2)})\neq \supp(\xstar)$.
This implies that $M$ does not have a unique Nash equilibrium, which is a contradiction.
Therefore, $V_{M_1}<V_{M}$.
\end{proof}

Analogously, one can also prove the following lemma.
\begin{lemma}\label{lem:ne->psne:2}
Consider a matrix $M\in \bbR^{k\times n}$. Let $M$ have a unique Nash equilibrium $(\xstar,\ystar)$ such that $|\supp(\ystar)|=k$.
Consider a $k\times k$ submatrix $M_1$ of $M$ with column indices $\calJ$.
If $\calJ\neq \supp(\ystar)$ then $V_{M_1}^\star>V_M^\star$. 
\end{lemma}

Recall that due to \Cref{Unique-NE-submatrix}, any submatrix $M$ of $A$ containing the row indices $\supp(\xstar)$ and column indices $\supp(\ystar)$ has a unique Nash equilibrium $(\xhat,\:\yhat)$ such that $\supp(\xhat)=\supp(\xstar)$ and $\supp(\yhat)=\supp(\ystar)$.
Moreover, $V_M^\star=V_A^\star$.
Let $\istar=f^{-1}(\supp(\xstar))$ and $\jstar=f^{-1}(\supp(\ystar))$. Now, observe that $A^{(k)}_{\istar,\jstar}=V_A^\star$.
By applying \Cref{lem:ne->psne:1} on the submatrix of $A$ with row indices $[n]$ and column indices $\supp(\ystar)$ and \Cref{lem:ne->psne:2} on the submatrix of $A$ with row indices $\supp(\xstar)$ and column indices $[n]$ we get $A^{(k)}_{i,\jstar}<A^{(k)}_{\istar,\jstar}<A^{(k)}_{\istar,j}$ for all $i\neq \istar$ and $j\neq \jstar$.
By applying \Cref{Unique-PSNE}, we get that $A^{(k)}$ has a unique PSNE $(\istar,\jstar)$.

Due to \Cref{lem:psne-correct}, we know that \psnealg/($A^{(k)}$) returns the unique PSNE $(\istar,\jstar)$ with probability at least $1-\delta$. Hence, our randomized procedure correctly returns the unique Nash equilibrium with probability at least $1-\delta$. Next, we establish the query complexity of $\psnealg/(A^{(k)})$. 

\begin{lemma}\label{lem:msne-query}
The algorithm \psnealg/$(A^{(k)})$ queries $O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ entries of the matrix $A$.
\end{lemma}

\begin{proof}
Recall that at each iteration $t$ of \psnealg/($A^{(k)}$), we maintained sets $\calX_t$, $\calY_t$, $\Xbar_t$, and $\Ybar_t$ and queried the entries of $A^{(k)}$ in the sets $\{(i,j):i\in\calX_t,j\in \Ybar_t\}$ and $\{(i,j):i\in \Xbar_t,j\in \calY_t\}$.
Using our query model $\calQ$, we can query the entries in these sets by querying at most $2k\cdot n \cdot 2\log(\frac{2n^{2k}}{\delta})\leq 8n\cdot k^2\cdot \log(\frac{2n}{\delta})$ entries from $A$.
This is due to the fact that $\max\{|\Xbar_t|,|\Ybar_t|\}\leq 2\log(\frac{2n^{2k}}{\delta})$. Also recall that we computed indices $\ihat, \jhat$ and queried the entries of $A^{(k)}$ in the sets $\{(\ihat,j):j\in \calY_t\}$ and $\{(i,\jhat):i\in \calX_t\}$.
Again, using our query model $\calQ$, we can query the entries in these sets by querying at most $2kn$ entries from $A$. Now, observe that \psnealg/($A^{(k)}$) terminates in $t_\star\leq k\cdot \log(n)+1$ iterations.
Hence, \psnealg/($A^{(k)}$) queries at most $O(nk^3\cdot \log n\cdot\log(\frac{n}{\delta}))$ entries of matrix $A$.
\end{proof}

It is straightforward to relax the assumption on the knowledge of $|\supp(\xstar)|$. 
Indeed, given a pair $(x,y)$ such that $\max\{|\supp(x)|,|\supp(y)|\}=s$, we require $2ns$ entries of $A$ to verify whether it is a Nash equilibrium of $A$ or not.
Beginning with $s=1$, we call the procedure \psnealg/($A^{(s)}$) and compute a pair $(x,y)$ as described above using $O(ns^3\cdot \log n\cdot \log(\frac{n}{\delta}))$ queries from $A$, and we verify whether $(x,y)$ is a Nash equilibrium using $2ns$ entries. If it is not, then we increment $s$ by one and repeat the process.
This process terminates with probability $1-\delta$ when $s=k$. Hence, with probability $1-\delta$, the total number of queries taken from $A$ is at most $k\cdot O(nk^3\cdot \log n\cdot \log(\frac{n}{\delta}))=O(nk^4\cdot \log n\cdot \log(\frac{n}{\delta}))$.

\textbf{Remark 2:} When $k=o\left(\frac{n^{1/4}}{\sqrt{\log n}}\right)$, then with high probability, our algorithm computes the exact Nash Equilibrium by querying $o(n^2)$ entries from the input matrix.

% \begin{figure}[ht!]
% \centering
% \includegraphics[width=0.75\textwidth]{graphics/msne.pdf}
% \caption{The yellow sub-matrix in $A$ corresponds to the orange entry in $A^{(2)}$. It can be easily shown that $A$ has a unique Nash Equilibrium $(\xstar,\ystar)$ with $\supp(\xstar)=\{3,4\}$ and $\supp(\ystar)=\{1,2\}$. This implies that the orange entry in $A^{(2)}$ is the unique PSNE which is indeed the case. }
% \label{fig:msne}
% \end{figure}

%\textbf{Clever Sampling}: Suppose we want to sample $\log(m^k)$ elements from each row of $B$ such that an event $G$ holds w.h.p. We can achieve the same goal by first choosing $\log(m^k)$ column indices of $B$ and then see all the entries in these columns. This corresponds to see all the entries of columns of $A$ that are associated with these  $\log(m^k)$ column indices which are at most $k\cdot \log(m)$ as each column of $B$ is associated with exactly $k$ columns of $A$. Hence the total number of samples used is $n\cdot k\cdot \log(m)$. We can use union bound to show that event $G$ holds w.h.p.

==> randomized_psne_alg.tex <==
\section{An Upper Bound for Finding the Nash Equilibrium}\label{sec:upper}
%\textcolor{red}{

\textcolor{red}{Decide later if you require this motivation or not.}

First, we would like to highlight a major challenge in designing a randomized algorithm for finding the unique Nash equilibrium $(\xstar,\ystar)$.
To do so, let us consider the case when the input matrix has a unique PSNE.
In order to design an algorithm whose query complexity is independent of any matrix-dependent gap parameter, we cannot make decisions based on linear combinations of entries of the matrix like the standard no-regret algorithms (see Appendix \ref{appendix:upper} for more details).

However, in order to  determine whether an entry $(i,j)$ is the unique PSNE, we only need to compare the entry with the other entries in its row and other entries in its column.
This observation suggests that one way to avoid a gap dependence is to design an algorithm that is based solely on comparing individual entries of the matrix.
To this end, we design \Cref{alg:psne}, \psnealg/, which, independent of any gap parameter, requires $O(n\log (\frac{n}{\delta}))$ queries to find the unique PSNE with probability $1-\delta$.
Moreover, Algorithm~\ref{alg:psne} has an additional property that the entries of the input matrix can take arbitrary real values, which is generally not the case with the no-regret algorithms.

%}

%\textcolor{red}{
In order to address the the challenge of avoiding gap dependence in the case when $k:=|\supp(\xstar)|\geq 2$, we construct a matrix $A^{(k)}$ based on the input matrix $A$ such that $A^{(k)}$ has a unique PSNE corresponding to the support of the Nash equilibrium of $A$; we can then run \Cref{alg:psne} on $A^{(k)}$.
Note that we present a deterministic algorithm in \Cref{sec:deterministic}, \sword/, which finds the unique PSNE in $O(n)$ queries.
However, due to its reliance on querying diagonal entries of the input matrix in an iterative manner, running \sword/ on $A^{(k)}$ would lead to a query complexity of $\Omega(n^2)$.
We address this issue in the construction of \Cref{alg:psne} to avoid a query complexity of $\Omega(n^2)$ when run on matrix $A^{(k)}$.
%}


\subsection{A Randomized Algorithm to Find the Unique 
PSNE}\label{sec:random:psne}

\textcolor{red}{Convert this into a sub-routine for a matrix $M\in\mathbb{R}^{n\times m}$. Maybe also mention that with an oracle access of rows and columns only. Also do the analysis for non-unique PSNE case.}

In this section, we assume that the input matrix $A\in\bbR^{n\times n}$ has a unique PSNE $(\istar,\jstar)$.
Due to \Cref{Nash-Shapley-lemma}, we have that $A_{i,\jstar}<A_{\istar,\jstar}<A_{\istar,j}$ for all $i\in [n]\setminus \{\istar\}$ and $j\in[n]\setminus \{\jstar\}$.
We use this crucial fact to design a randomized algorithm, \psnealg/  (\Cref{alg:psne}), for finding a unique PSNE. We first state our main result below.
%\ross{We should have a better way to write these double inequalities without the ``holds for all $i\in [m]\setminus \{\istar\}$ and $j\in[n]\setminus \{\jstar\}$" stuff, it's really cumbersome. I think ``for all $i\neq\istar,j\neq\jstar$" may be good enough if just saying for all $(i,j)$ is gonna annoy someone, but even that I think might be OK.}

%\ross{I'm not sure why the lines I commented out would be needed: We are assuming a PSNE, so if you verify one, you're done. We don't need to reason about another one. Am I missing something?}
%\arnab{Read the proof of deterministic algorithm to see why they are required. We don't want a scenario where multiple elements satisfy the strict inequality in some submatrix. This would be problematic. Or in other words, I want to claim the $(\istar,\jstar)$ is the unique PSNE of any submatrix it is part of. I am undoing the commenting of the lines.}
% Hence, we would require at most $n_1+m_1$ queries to verify whether $(\istar,\jstar)$ is a unique PSNE of $B$ or not

%Thus, If we want to verify if a pair $(\istar,\jstar)$ is a unique PSNE of $B\in\bbR^{n_1\times m_1}$, it suffices to check whether $M_{i,\jstar}<M_{\istar,\jstar}<M_{\istar,j}$ holds for all $i\in [n_1]\setminus \{\istar\}$ and $j\in[m_1]\setminus \{\jstar\}$, which requires $n_1+m_1$ queries.

% Therefore, if we want to verify if a pair $(\istar,\jstar)$ is a unique PSNE of $B\in\bbR^{n_1\times m_1}$ or not, it just suffices to check whether $B_{i,\jstar}<B_{\istar,\jstar}<B_{\istar,j}$ holds for all $i\in [n_1]\setminus \{\istar\}$ and $j\in[m_1]\setminus \{\jstar\}$ or not.
% Hence, we would require at most $n_1+m_1$ queries to verify whether $(\istar,\jstar)$ is a unique PSNE of $B$ or not.

%\textcolor{red}{ARNAB: I have used $A_{i,j}$ to denote the element $(i,j)$ at many places. I will change it sometime later.}
% \begin{figure}[ht]
% \centering
% 	\includegraphics[width=0.3\linewidth]{graphics/psne.png}
%  \caption{Recursively dividing the input matrix}
% \end{figure}

%\textcolor{red}{ARNAB: Will remove Figure 1 most probably.}
%\subsection{Randomized Algorithm for finding PSNE}
%\arnab{Ignore the first paragraph below. You can read rest of the stuff.}

% Recall that any randomized algorithm for finding the unique PSNE has a lower bound of $\Omega(n)$ on the query-complexity. 
% On the other hand, we showed that there is a deterministic algorithm that queries $O(n^{\log_23})$ entries of the input matrix $A$ and returns the unique PSNE $(\istar,\jstar)$. This leads us to the following question: Is there a randomized algorithm that queries at most $O(n\cdot \text{poly}\log(n))$ queries from the input matrix in the worst case and returns the unique PSNE with high probability. We answer this question affirmatively in the following theorem.

\begin{theorem}\label{thm:psne}
\psnealg/ (\Cref{alg:psne}) queries at most $O(n\log(\frac{n}{\delta}))$ entries of the input matrix $A\in\bbR^{n\times n}$ and returns the unique PSNE $(\istar,\jstar)$ with probability at least $1-\delta$.
\end{theorem}


% In this section, we repeatedly use the following lemma:
% \begin{lemma}\label{tradeoff:lem}
% Consider the matrix $A\in\bbR^{n_1\times m_1}$ and two constants $c_1,c_2$ such that $1\leq c_1<c_2\leq\min\{n_1,m_1\}$. Let $x\in\bbR$. Let $\calC$ be the set of columns such that the number of elements less than $x$ in each of these columns is at least $n_1(1-\frac{1}{c_2})$. Let $\calR$ be the set of rows such that the number of elements more than $x$ in each of these rows is at least $m_1(1-\frac{1}{c_2})$. The following holds true:
% \begin{itemize}
%     \item If $|\calC|\geq \frac{m_1}{c_1}$, then $|\calR|\leq \frac{2n_1}{c_2-c_1}$
%      \item If $|\calR|\geq \frac{n_1}{c_1}$, then $|\calC|\leq \frac{2m_1}{c_2-c_1}$
% \end{itemize}
% \end{lemma}
% \begin{proof}
% Let $|\calC|\geq \frac{m_1}{c_1}$. Consider a subset $\calC'\subset \calC$ such that $|\calC'|= \lceil\frac{m_1}{c_1}\rceil$. Let $A_1$ be the sub-matrix of $A$ with all the $n_1$ rows and the columns being the set $\calC'$. Now the number of elements of $A_1$ less than $x$ is at least $\lceil \frac{m_1}{c_1}\rceil\cdot n_1\left(1-\frac{1}{c_2}\right)$. Hence, the number of elements of $A_1$ more than $x$ is at most $\lceil \frac{m_1}{c_1}\rceil\cdot \frac{n_1}{c_2}\leq \frac{2n_1m_1}{c_1c_2}$. We get the last inequality as for all $x\geq 1$, $\lceil x\rceil \leq 2x$.

% Now consider the set $\calR$. Let $A_2$ be the sub-matrix of $A$ with all the $m_1$ columns and the rows being the set $\calR$. Number of elements of $A_2$ that are not in the submatrix $A_1$ is at most $|\calR|\cdot m_1(1-\frac{1}{c_1})$. Hence the number of elements of $A_2$ that are more than $x$ and are not in the submatrix $A_1$ is at most $|\calR|\cdot m_1(1-\frac{1}{c_1})$. Now the number of elements of $A_2$ more than $x$ is at least $|\calR|\cdot m_1 \left(1-\frac{1}{c_2}\right)$. Hence the number of elements of $A_2$ that are more than $x$ and are in the submatrix $A_1$ is at least $|\calR|\cdot m_1(\frac{1}{c_1}-\frac{1}{c_2})$. Recall that the number of elements of $A_1$ more than $x$ is at most $\frac{2n_1m_1}{c_1c_2}$. Therefore, we have $|\calR|\cdot m_1(\frac{1}{c_1}-\frac{1}{c_2})\leq \frac{2n_1m_1}{c_1c_2}$ which implies that $|\calR|\leq \frac{2n_1}{c_2-c_1}$. By using similar arguments one can show that if $|\calR|\geq \frac{n_1}{c_1}$, then $|\calC|\leq \frac{2m_1}{c_2-c_1}$.
% \end{proof}

% \begin{corollary}\label{tradeoff:cor}
% Consider the matrix $A\in\bbR^{n_1\times m_1}$ and a positive constant $c$ such that $1\leq c\leq\min\{n_1,m_1\}$. Let $x\in\bbR$. Let $\calC$ be the set of columns such that the number of elements less than $x$ in each of these columns is at least $n_1(1-\frac{1}{3c})$. Let $\calR$ be the set of rows such that the number of elements more than $x$ in each of these rows is at least $m_1(1-\frac{1}{3c})$. The following holds true:
% \begin{itemize}
%     \item If $|\calC|\geq \frac{m_1}{c}$, then $|\calR|\leq \frac{n_1}{c}$
%      \item If $|\calR|\geq \frac{n_1}{c}$, then $|\calC|\leq \frac{m_1}{c}$
% \end{itemize}
% \end{corollary}
% \begin{proof}
%     We get the result in the corollary by substituting $c_1=c$ and $c_2=3c$ in the lemma \ref{tradeoff:lem}.
% \end{proof}

% \arnab{Let's keep \Cref{thm:psne} in this section only. Because this section is exclusively for unique PSNE. Would be confusing otherwise. The previous section was just to highlight the technical challenges (and not to summarize our contributions as such)}

\begin{algorithm2e}[!ht]
\caption{\psnealg/($A$)}
\label{alg:psne}
\DontPrintSemicolon
$n\gets$ number of rows of $A$,\: $\calX_1 \gets [n], \:\calY_1 \gets [n]$\;
\For{$t=1,2,\ldots$}{
    \If{$|\calX_t|=1$}{
    \KwRet $(\;\ihat,\:\jhat\;)$, where $\calX_t=\{\;\ihat\;\}$ and $\calY_t=\{\;\jhat\;\}$
    }
    $n_t\gets |\calX_t|$ and $\ell\gets 2\log(\frac{2n^2}{\delta})$\;
    $\Xbar_t \gets\{x_1,x_2,\ldots, x_{\ell}\}$; $x_i$'s are drawn independently and uniformly at random from $\calX_t$ \label{recurse:line2}\;
    $\Ybar_t \gets \{y_1,y_2,\ldots, y_{\ell}\}$; $y_j$'s are drawn independently and uniformly at random from $\calY_t$ \label{recurse:line3}\;
    Query all the entries of $A$ in $\{(i,j):i\in\calX_t,j\in \Ybar_t\}\cup\{(i,j):i\in \Xbar_t,j\in \calY_t\}$\;
    
    %Query each $(i\:,j)$ in $\{\calX_t \times \Ybar_t\} \cup \{\Xbar_t\times  \calY_t\}$\;
    Choose the arguments $\ihat\in \argmax_{i\in\calX_t}\min_{j\in \Ybar_t}A_{i,j}$ and $\jhat\in \argmin_{j\in\calY_t}\max_{i\in \Xbar_t}A_{i,j}$\;
    Query all the entries of $A$ in $\{({i,\jhat}): i\in \calX_t\}\cup\{({\ihat,\:j}):j\in\calY_t\}$\;
    
    %Query each $(i,j)$ in $\{\calX_t \times \jhat\} \cup \{\ihat \times \calY_t\}$\;
    %\tcp{Sort Xt by j\_hat and Yt by i\_hat, take half}
    $\calX_{t+1}\gets \{i_1,i_2,\ldots, i_{\lfloor n_t/2\rfloor}\} \subseteq \calX_t=\{i_1,\ldots,i_{n_t}\}$,   where $A_{i_1,\jhat}\geq A_{i_2,\jhat}\geq \ldots \geq A_{i_{n_t},\jhat}$\;
    $\calY_{t+1}\gets \{j_1,j_2,\ldots, j_{\lfloor n_t/2\rfloor}\}\subseteq \calY_t=\{j_1,\ldots,j_{n_t}\}$, where $A_{\ihat,j_1}\leq A_{\ihat,j_2}\leq \ldots \leq A_{\ihat,j_{n_t}}$\;
}
\end{algorithm2e}

\textbf{Remark 1:} The case of $n\times m$ matrix is subsumed in the case of $n\times n$ matrix as one can pad the matrix with dummy elements to convert it into a $n\times n$ matrix, assuming $n\geq m$. However, one can easily modify the above algorithm to address the case of $n\times m$. We refer the reader to \Cref{appendix:modification-psne} for this modified procedure called \psnealg/2($A$) which has the same guarantees as \psnealg/($A$).

We now begin the proof of \Cref{thm:psne} with the following proposition.

\begin{proposition}\label{lem:probability-bound}
Fix $c,k\in \bbN$ with $k\geq 3$.
Consider a set $S=\{a_1,a_2,\ldots,a_{k}\}$, and let $S_1=\{a_1,a_2,\ldots, a_{\lfloor k/2\rfloor}\}$.
Let $\ell=2\log (\frac{c}{\delta})$, and let $X=\{x_1,x_2,\ldots,x_\ell\}$ where $x_i$'s are drawn independently and uniformly at random from $S$.
Then, $X\cap S_1 \neq \emptyset$ with probability at least $1-\frac{\delta}{c}$.
\end{proposition}
\begin{proof} As the events $\{x_i \notin S_1\}$ are independent,
\begin{align*}
\bbP(X\cap S_1 = \emptyset) = \prod_{i=1}^\ell \bbP(x_i \notin S_1) = \Par*{\tfrac{k-\lfloor k/2 \rfloor}{k}}^\ell \leq \Par*{\tfrac{2}{3}}^{2\log (\frac{c}{\delta})}<\tfrac{\delta}{c}.
\end{align*}
\end{proof}

We now establish the query complexity of \psnealg/ in the following lemma.
\begin{lemma}\label{lem:psne-query}
\psnealg/$(A)$ queries at most $8n\log(\frac{4n^2}{\delta})$ entries of $A$.
\end{lemma}
\begin{proof}
Iteration $t$ requires at most $2\ell n_t+2n_t$ queries.
Since $n_t\leq\frac{n}{2^{t-1}}$, we have that $\sum_{t=1}^\infty n_t\leq 2n$.
Hence, the total number of queries is at most $2n(2\ell+2) \leq 8n\log(\frac{4n^2}{\delta})$.
\end{proof}

Finally, we establish the correctness of \psnealg/ in the following lemma.
\begin{lemma}\label{lem:psne-correct}
\psnealg/$(A)$ returns the unique PSNE with probability at least $1-\delta$.
\end{lemma}

\begin{proof}
Recall that $(\istar,\jstar)$ is the unique PSNE of $A$.
Assume that $\istar\in\calX_t$ and $\jstar\in\calY_t$ at some iteration $t$. 
We will show that $\istar\in\calX_{t+1}$ and $\jstar\in\calY_{t+1}$ with probability at least $1-\frac{\delta}{n}$. 
    
For each $j\in \calY_t$, let us relabel the indices in $\calX_t$ as $\{i_1,i_2,\ldots,i_{n_t}\}$ such that $A_{i_1,j}\geq A_{i_2,j}\geq\ldots\geq A_{i_{n_t},j}$ and let $\calR_{t,j}:=\{i_1,i_2,\ldots,i_{\lfloor n_t/2\rfloor}\}$. 
Recall that $\Xbar_t$ and $\Ybar_t$ are random subsets of $\calX_t$ and $\calY_t$ respectively. By \Cref{lem:probability-bound} we have $\mathbb{P}(\Xbar_{t}\cap \calR_{t,j}\neq \emptyset)\geq 1-\frac{\delta}{2n^2}$ for a fixed $j$.
By the union bound, we then have that with probability at least $1-\frac{\delta}{2n}$, the event $\calE_t:=\{\Xbar_t\cap \calR_{t,j}\neq \emptyset \:\forall \:j\in\calY_t\}$ holds. Note that if $\calE_t$ holds, for each $j\in\calY_t$ we have $\argmax_{i\in\Xbar_t}A_{i,j}\cap \calR_{t,j}\neq \emptyset$.

Assume $\calE_t$ holds, and let $v^\star_y=\min_{j\in\calY_t}\max_{i\in \Xbar_t}A_{i,j}$. Recall that $\jhat\in \arg\min_{j\in\calY_t}\max_{i\in \Xbar_t}A_{i,j} $. If $\jhat=\jstar$, then $\istar\in  \calR_{t,\jhat}=\calX_{t+1}$, as $A_{\istar,\jstar}$ is the unique highest element of column $\jstar$. Next, let us consider the case where $\jhat\neq \jstar$.
As $\calE_t$ holds, $\argmax_{i\in \Xbar_t}A_{i,\jhat}\cap \calR_{t,\jhat}\neq \emptyset$.
We also see that 
$v^\star_y = \min_{j\in\calY_t}\max_{i\in \Xbar_t}A_{i,j} \leq \max_{i\in \Xbar_t}A_{i,\jstar}\leq A_{\istar,\jstar}$. Recall that for all $j\in\calY_t\setminus\{\jstar\}$, we have $A_{\istar,j}> A_{\istar,\jstar}$.
Now for all $i\in \calX_t\setminus \calR_{t,\jhat}$, we have $A_{i,\jhat}\leq v_y^\star\leq  A_{\istar,\jstar}<A_{\istar,\jhat}$. Hence, $\istar \in \calR_{t,\jhat}=\calX_{t+1}$.

By an identical argument, we have $\jstar\in \calY_{t+1}$ with probability at least $1-\frac{\delta}{2n}$.
Hence, by the union bound, with probability at least $1-\frac{\delta}{n}$ we have $\istar\in\calX_{t+1}$ and $\jstar\in\calY_{t+1}$.
Observe that the algorithm terminates at a fixed iteration $t_\star$ which is at most $\log(n)+1$.
Now observe that \psnealg/$(A)$ returns $(\istar,\jstar)$ if $\istar\in\calX_{\tstar}$ and $\jstar\in\calY_{\tstar}$.
Let $p_t=\bbP(\istar\in \calX_{t},\jstar\in\calY_t|\istar\in \calX_{t-1},\jstar\in\calY_{t-1})$.
Now we have the following due to the chain rule and Bernoulli's inequality,
 \begin{equation*}
     \bbP(\istar\in\calX_{\tstar},\jstar\in\calY_{\tstar})=\prod_{t=2}^{t_\star}p_t\geq \left(1-\frac{\delta}{n}\right)^{t_\star}\geq 1-\delta.
 \end{equation*}
% where the last inequality follows from the fact that $(1+x)^r\geq 1+rx$ for all $x\geq -1$ and $r\geq 2$.
\end{proof}



\Cref{thm:psne} follows directly from \Cref{lem:psne-query} and \Cref{lem:psne-correct}.

%\textbf{Remark:} Observe that unlike no-regret algorithms, Algorithm~\ref{alg:psne}'s query complexity bound does not depend on any matrix dependent gap parameters. Moreover, Algorithm~\ref{alg:psne} does not require the entries of the matrix to be bounded between $-1$ and $1$. Instead, the entries of the matrix can take arbitrary real values. 
% \textbf{Open Question:} Can we design a logarithmic stage based algorithm that uses sublinear queries and finds the suport of the Mixed Nash equilibrium?

% \noindent 
% \textbf{Answer:} Yes. See next section.

% \subsection{Ideas for $n\log n$ randomized algorithm}
% In the previous subsection, the bounds depended on the gap parameter $\simplex_g$. It remains an open question whether we can obtain a bound of $O(n\log n)$ that is independent of any gap parameter. It appears that one should be able to design an algorithm based on comparisons only. Anything on top of this (like summing the values of a row) will naturally lead to bound that involves the gap parameters. 


% \textbf{Idea 1:} One idea to resolve this issue is to take the following approach. First we do a computation row wise. For each element $(i,j)$ in row $i$, we compute the number of elements in the column $j$ that are less than the element $(i,j)$. Let this value be $w_{ij}$. Next  we do a computation column wise. For each element $(i,j)$ in column $j$, we compute the number of elements in the row $i$ that are more than the element $(i,j)$. Let this value be $v_{ij}$. Recall that $(\istar,\jstar)$ is the unique PSNE. Now we have the following:
% \begin{equation*}
%     \sum_{j\in[m]}w_{\istarj}+\sum_{i\in[n]}v_{i\jstar}\approx n\cdot m
% \end{equation*}
% This implies that either $\sum_{j\in[m]}w_{\istarj}\geq nm/2$ or $\sum_{i\in[n]}v_{i\jstar}\geq nm/2$. Now if we want to reduce the size of the input matrix by a factor and retain either the optimal column $\jstar$ or the optimal row $\istar$. One might consider the idea of retaining only those rows $i'$ and columns $j'$ for which the values $ \sum_{j\in[m]}w_{i'j}$ and $\sum_{i\in[n]}v_{ij'}$ are high. However there exists a matrix for which this value is roughly equal to $nm/2$ for all rows and columns. However the optimal row and column have an additional structural property. The elements of the optimal row is less than a certain value (which is $V_A^\star$) and the elements of the optimal column is greater than a certain value (which is $V_A^\star$). So in order to capture this structural property, some additional regularizing term might be required. For instance, one might try to retain those rows $i$ and columns $j$ for which the following values are high:
% \begin{align*}
%     \bar w_i-\frac{1}{2}||w_i-{\bf\bar w_i}||^2\\
%     \bar v_j-\frac{1}{2}||v_j-{\bf\bar v_j}||^2\\
% \end{align*}
% Here $w_i$ denotes the vector $(w_{i,1},w_{i,2},\ldots,w_{i,m})^T$, $v_j$ denotes the vector $(v_{1,j},w_{2,j},\ldots,w_{n,j})^T$, $\bar w_i=\frac{1}{m}\cdot\sum_{j=1}^mw_{ij}$, $\bar v_j=\frac{1}{n}\cdot\sum_{i=1}^nv_{ij}$, ${\bf\bar w_i}$ denotes the $m$-dimensional vector $(\bar w_i,\ldots,\bar w_i)$ and ${\bf\bar v_j}$ denotes the $n$-dimensional vector $(\bar v_j,\ldots,\bar v_j)$. It remains a challenge to show that this regularizer (or any other regularizer) manages to reduce the size of the matrix by a constant factor and either retain the optimal row or the optimal column. 

==> randomized_psne_alg_old.tex <==


\begin{algorithm}[!ht]
\caption{\textsc{PSNE}($A,n$)}

\label{alg:psne}
\begin{algorithmic}[1]
%\REQUIRE Value of the game $V_A^\star$
\STATE Let $\calX_1$ be the row indices of $A$ and $\calY_1$ be the column indices of $A$
\FOR{$t=1,2,\ldots$}
\STATE If $|\calX_t|=1$, \textbf{return} $(\;\ihat,\jhat\;)$ where $\calX_t=\{\;\ihat\;\}$ and $\calY_t=\{\;\jhat\;\}$
\STATE $n_t\gets |\calX_t|$ and $\ell\gets 2\log(\frac{2n^2}{\delta})$
\STATE Construct a set $X_{1,t}=\{x_1,x_2,\ldots, x_{\ell}\}$ where each $x_i$ is sampled independently and 
uniformly at random from $\calX_t$. Let $X_{2,t}$ be the set of unique elements of $X_{1,t}$. \label{recurse:line2}
\STATE Construct a set $Y_{1,t}=\{y_1,y_2,\ldots, y_{\ell}\}$ where each $y_i$ is sampled independently and 
uniformly at random from $\calY_t$. Let $Y_{2,t}$ be the set of unique elements of $Y_{1,t}$. \label{recurse:line3}
\STATE Query all the entries of $A$ in the sets $\{(i,j):i\in\calX_t,j\in Y_{2,t}\}$ and $\{(i,j):i\in X_{2,t},j\in \calY_t\}$
%\STATE For each $i\in \calX$, let $u_i$ be the smallest element of the set $\{A_{i,j}:j\in Y_2\}$
\STATE $\ihat\gets \argmax_{i\in\calX_t}\min_{j\in Y_{2,t}}A_{i,j}$ and $\jhat\gets \argmin_{j\in\calY_t}\max_{i\in X_{2,t}}A_{i,j}$
%\STATE For each $j\in \calY$, let $v_j$ be the largest element of the set $\{A_{i,j}:i\in X_2\}$
\STATE Query all the entries of $A$ in the sets $\{({i,\jhat}): i\in \calX_t\}$ and $\{({\ihat,j}):j\in\calY_t\}$.
\STATE Let us label the elements of $\calX_t$ as $\{i_1,i_2,\ldots, i_{n_t}\}$ where $A_{i_1,\jhat}\geq A_{i_2,\jhat}\geq \ldots \geq A_{i_{n_t},\jhat}$
\STATE Let us label the elements of $\calY_t$ as $\{j_1,j_2,\ldots, j_{n_t}\}$ where $A_{\ihat,j_1}\leq A_{\ihat,j_2}\leq \ldots \leq A_{\ihat,j_{n_t}}$
\STATE $\calX_{t+1}\gets \{i_1,i_2,\ldots, i_{\lfloor n_t/2\rfloor}\}$ and $\calY_{t+1}\gets \{j_1,j_2,\ldots, j_{\lfloor n_t/2\rfloor}\}$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

% \textbf{Remark}: There are two parts for the analysis. Using Corollary \ref{tradeoff:cor} and chernoff bound, we can show that with high proability either the size of $\calX$ or $\calY$ gets reduced by a factor of $\frac{1}{2}$ in every iteration of the while loop. Also we can show that with high probability, the PSNE $(\istar,\jstar)$ does not get sampled in the while loop. This ensures that that $\istar\in \calX$ and $\jstar\in\calY$ in each iteration of the while loop.

%  Via a similar recursive procedure we can find PSNE by querying at most $O(n^{1+o(1)})$ elements of $A$. The main difference is that an $n\times n$ matrix is recursively divided into an $\frac{n}{\log n}\times n $ matrix and an $n\times\frac{n}{\log n}$ matrix in such a way that optimal row or column lies in one of these matrices. This can be achieved using the property mentioned in the Corollary \ref{tradeoff:cor}. We extend this idea in the next section. 



\begin{proof}
Let $(\istar,\jstar)$ be the PSNE of $A$.
Assume that $\istar\in\calX_t$ and $\jstar\in\calY_t$ at some iteration $t$. 
We will show that $\istar\in\calX_{t+1}$ and $\jstar\in\calY_{t+1}$ with probability at least $1-\frac{\delta}{n}$. 
    
For each $j\in \calY_t$, let us relabel the indices in $\calX_t$ as $\calR_{1,j}:=\{i_1,i_2,\ldots,i_{n_t}\}$ such that $A_{i_1,j}\geq A_{i_2,j}\geq\ldots\geq A_{i_{n_t},j}$ and let $\calR_{2,j}:=\{i_1,i_2,\ldots,i_{\lfloor n_t/2\rfloor}\}$. 
Recall the definition of $X_{2,t}$ and $Y_{2,t}$ in \Cref{alg:psne}.
Due to \Cref{lem:probability-bound}, with probability at least $1-\frac{\delta}{2n^2}$ we have $X_{2,t}\cap \calR_{2,j}\neq \emptyset$ for a fixed $j$.
By a union bound, with probability at least $1-\frac{\delta}{2n}$, we have that $X_{2,t}\cap \calR_{2,j}\neq \emptyset$ for all $j\in\calY_t$.


Let us assume that $X_{2,t}\cap \calR_{2,j}\neq \emptyset$ for all $j\in\calY_t$.
Let $v_y^\star=\min_{j\in\calY_t}\max_{i\in X_{2,t}}A_{i,j}$ and $\jhat= \argmin_{j\in\calY_t}\max_{i\in X_{2,t}}A_{i,j}$.
If $\jhat=\jstar$, then $\istar\in  \calR_{2,\jhat}=\calX_{t+1}$ as $A_{\istar,\jstar}$ is the unique highest element of column $\jstar$.
Now let us consider the case where $\jhat\neq \jstar$. First observe that $\argmax_{i\in X_{2,t}}A_{i,\jhat}\in \calR_{2,\jhat}$ due to our assumption.
Next observe that $\max_{i\in X_{2,t}}A_{i,\jstar}\leq A_{\istar,\jstar}$. Hence $v_y^\star\leq  A_{\istar,\jstar}$.
Next observe that for all $j\in\calY_t\setminus\{\jstar\}$, we have $A_{\istar,j}> A_{\istar,\jstar}$.
Now for all $i\in \calX_t\setminus \calR_{2,\jhat}$, we have $A_{i,\jhat}\leq v_y^\star\leq  A_{\istar,\jstar}<A_{\istar,\jhat}$. Hence, we have $\istar \in \calR_{2,\jhat}=\calX_{t+1}$. Analogously, using the same argument, we can show that with probability $1-\frac{\delta}{2n}$, we have $\jstar\in \calY_{t+1}$.
% %for each $i\in \calX_t$, let us relabel the indices in $\calY_t$ as $\calC_{1,i}:=\{j_1,j_2,\ldots,j_{n_t}\}$ such that $A_{i,j_1}\leq A_{i,j_2}\leq\ldots\leq A_{i,j_{n_t}}$ and let $\calC_{2,i}:=\{j_1,j_2,\ldots,j_{\lfloor n_t/2\rfloor}\}$.
% % Recall the definition of $X_{2,t}$ and $Y_{2,t}$ in Algorithm \ref{alg:psne}.
% % Due to Lemma \ref{lem:probability-bound}, with probability at least $1-\frac{\delta}{2n^2}$ we have that $Y_{2,t}\cap \calC_{2,i}\neq \emptyset$ for a fixed $i$.
% % Due to union bound, with probability at least $1-\frac{\delta}{2n}$ we have $Y_{2,t}\cap \calC_{2,i}\neq \emptyset$ for all $i\in\calX_t$. Let us assume that $Y_{2,t}\cap \calC_{2,i}\neq \emptyset$ for all $i\in\calX_t$.
% % Let $v_x^\star=\max_{i\in\calX_t}\min_{j\in Y_{2,t}}A_{i,j}$ and $\ihat= \argmax_{i\in\calX_t}\min_{j\in Y_{2,t}}A_{i,j}$.
% % If $\ihat=\istar$, then $\jstar\in  \calC_{2,\ihat}=\calY_{t+1}$ as $A_{\istar,\jstar}$ is the unique lowest element of row $\istar$.
% % Now let us consider the case where $\ihat\neq \istar$. First observe that $\argmin_{j\in Y_{2,t}}A_{\ihat,j}\in \calC_{2,\ihat}$ due to our assumption.
% % Next observe that $\min_{j\in Y_{2,t}}A_{\istar,j}\geq  A_{\istar,\jstar}$. Hence $v_x^\star\geq  A_{\istar,\jstar}$.
% % Next observe that for all $i\in\calX_t\setminus\{\istar\}$, we have $A_{i,\jstar}< A_{\istar,\jstar}$.
% % Now for all $j\in \calY_t\setminus \calC_{2,\ihat}$, we have $A_{\ihat,j}\geq v_x^\star\geq  A_{\istar,\jstar}>A_{\ihat,\jstar}$. Hence, $\jstar \in \calC_{2,\ihat}=\calY_{t+1}$.
%  %\kevin{Isn't the above paragraph almost identical to the first, but just changing the direction (max to min)? Do you think we need to include it?}
% %\arnab{Not necessary. We can push it appendix.}
    
Hence, by a union bound, with probability at least $1-\frac{\delta}{n}$ we have $\istar\in\calX_{t+1}$ and $\jstar\in\calY_{t+1}$.
Observe that the algorithm terminates at a fixed iteration $t_\star$ which is at most $\log n+1$.
Now observe that \textsc{PSNE}$(A,n)$ returns $(\istar,\jstar)$ if $\istar\in\calX_{\tstar}$ and $\jstar\in\calY_{\tstar}$.
Let $p_t=\bbP[\istar\in \calX_{t},\jstar\in\calY_t|\istar\in \calX_{t-1},\jstar\in\calY_{t-1}]$.
Now we have the following due to the chain rule:
 \begin{equation*}
     \bbP[\istar\in\calX_{\tstar},\jstar\in\calY_{\tstar}]=\prod_{t=2}^{t_\star}p_t\geq \left(1-\frac{\delta}{n}\right)^{t_\star}\geq 1-\delta,
 \end{equation*}
where the last inequality follows from the fact that $(1+x)^r\geq 1+rx$ for all $x\geq -1$ and $r\geq 2$.
\end{proof}

==> swordfish.tex <==
\section{An \texorpdfstring{$\bigO(n \log n)$}{O(n log n)} Deterministic Algorithm to Find the Unique PSNE}\label{sec:deterministic}

In this section, we return to the setting in which  the input matrix $A\in\bbR^{n\times n}$ has a unique PSNE $(\istar,\jstar)$, and we
detail \sword/, a simple deterministic algorithm that finds the unique PSNE $(\istar,\jstar)$ in $\bigO(n\log n)$ queries.
By \Cref{Nash-Shapley-lemma}, the PSNE has positive row and column gaps. That is, 
% \begin{equation}
% A_{(1),\jstar}\leq \ldots \leq A_{(n-1),\jstar}< A_{(n),\jstar}=A_{\istar,\jstar} = A_{\istar,(1)} < A_{\istar,(2)} \leq \ldots \leq A_{\istar,(n)} . \label{eq:strict_gaps}
% \end{equation}
\begin{equation}
A_{i,\jstar}< A_{\istar,\jstar} < A_{\istar,j}\quad \forall i\in [n]\setminus\{\istar\},\: j\in[n]\setminus\{\jstar\} . \label{eq:strict_gaps}
\end{equation}
\subsection{\sword/ in theory}

The salient feature of  \textsc{Swordfish} is its adaptivity: it limits querying entries of $A$ that can be proven to not be the unique PSNE.

\begin{definition}
We call an entry $A_{i,j}$ \textbf{nullified} by entries $A_{i,\ell}$ and $A_{k,j}$ where $(i,\ell)\neq (k,j)$ if the two entries jointly contradict \eqref{eq:strict_gaps} for $(\istar,\jstar)=(i,j)$, i.e. if $A_{i,\ell}\leq A_{k,j}$ holds.
A nullified entry cannot be the unique PSNE of the matrix $A$.
\end{definition}

\sword/ is a recursive algorithm that proceeds as follows.
At each stage of the recursion (operating on $B\in\mathbb{R}^{m\times m}$, a submatrix of $A$ where $m$ is even), we first query the diagonal entries $B_{i,i}$ of $B$ and then permute the rows and columns of $B$ such that its diagonal entries are in non-decreasing order.
\textsc{Swordfish} relies almost exclusively on the insight that this diagonal sorting heavily constrains the location of the unique Nash equilibrium.
\begin{proposition}\label{lem:upper_tri}
If $B$ has non-decreasing entries along its diagonal, all entries of $B$ above the diagonal are nullified.
\end{proposition}
\begin{proof}
If $k<\ell$, $B_{k,\ell}$ is nullified by $B_{k,k}$ and $B_{\ell,\ell}$ as $B_{k,k}\leq B_{\ell,\ell}$.
% entry $(k,l)$ cannot be the unique PSNE of $B$; otherwise, \eqref{eq:strict_gaps} would imply
% $
% B_{k,l} < B_{k,k} \leq B_{l,l} < B_{k,l},
% $ which is a contradiction.
\end{proof}

At this point, we can immediately construct a $o(n^2)$ algorithm for finding the unique PSNE.
By standard recurrence analysis, finding the (at most one) unique PSNE of each of the three remaining $\frac{n}{2}\times \frac{n}{2}$ quadrants gives a query complexity of $\bigO(n^{\log_2 3}) \approx \bigO(n^{1.58})$.
However, by being more aggressive in marking entries as nullified at each stage, we can reduce the number of remaining subproblems from three to two.
To do so, we use the following core proposition, which gives a guarantee on being able to mark multiple entries as nullified with a single query.

\begin{proposition}\label{cor:core_movement}
Assume the diagonal entries of $B$ are known and non-decreasing, and fix $m\geq i >m/2\geq j \geq 1$, where $m\geq 2$.
If $B_{i,j}$ is queried, then at least one of the following statements is true:
\begin{enumerate}[label=(\alph*),itemsep=-1pt, topsep=2pt]
    \item we can mark $B_{j,j},\ldots,B_{m/2,j}$ as nullified, or
    \item we can mark $B_{i,m/2 + 1},\ldots,B_{i,i}$ as nullified.
\end{enumerate}
\end{proposition}
\begin{proof}
If $B_{i,j}\geq B_{m/2,m/2}$, then $B_{i,j}$ and $B_{\ell,\ell}$ nullify $B_{\ell,j}$ for $j\leq \ell \leq m/2$ as $B_{i,j} \geq B_{m/2,m/2} \geq  B_{\ell,\ell} $.
If $B_{i,j}\leq B_{m/2,m/2}$, then $B_{i,j}$ and $B_{k,k}$ nullify $B_{i,k}$ for $m/2+1\leq k \leq i$ as $B_{i,j} \leq B_{m/2,m/2} \leq  B_{k,k} $
\end{proof}
Thus, for each query point, either the first $m/2$ entries in its column or last $m/2$ entries in its row are nullified, by a combination of nullifying at or below the diagonal (\Cref{cor:core_movement}) and nullifying above the diagonal (\Cref{lem:upper_tri}).
\Cref{fig:core_prop} illustrates this fact, taking $B_{i,j}=B_{m,1}$ as an example.
\begin{figure}[ht!]
\centering
\includegraphics[width=0.98\textwidth]{graphics/swordfish_ex_flanked.pdf}
\caption{Three examples illustrating \Cref{cor:core_movement} when $B_{i,j}=B_{m,1}$ with $m=8$. With the diagonal of $B$ known and sorted, based on $B_{m,1}$ one can mark at least $m/2$ entries of either the last row or the first column of $B$ as nullified. The red cells have just been nullified, whereas the gray cells have already been marked as nullified via \Cref{lem:upper_tri}. The red dashed box surrounds the lower-left quadrant of $B$. \\ In the first example, $B_{4,1}$ is nullified by $B_{8,1}$ and $B_{4,4}$, as $9.1 < B_{4,1} < 4$ cannot hold.
}
\label{fig:core_prop}
\end{figure}

\Cref{cor:core_movement} now gives the core logic for \sword/: starting at $B_{i,j}=B_{m,1}$, we query $B_{i,j}$ and mark entries as nullified using \Cref{cor:core_movement}, and then move
\begin{itemize}[itemsep=-1pt, topsep=2pt]
    \item right (i.e. $B_{i,j+1}$), if \Cref{cor:core_movement}(a) holds,
    \item up (i.e. $B_{i-1,j}$), if \Cref{cor:core_movement}(b) holds, and
    \item diagonally up-right (i.e. $B_{i-1,j+1}$), if \Cref{cor:core_movement}(a) and \Cref{cor:core_movement}(b) both hold.
\end{itemize}
For example, after marking nullified entries in each example shown in \Cref{fig:core_prop}, the moves would be right, up, and up-right, respectively.
Upon exiting the lower-left quadrant, we will have successfully completed our objective: eliminating one of the three remaining subproblems.

\begin{proposition}\label{cor:sword_exit}
Starting at $B_{m,1}$, repeat the process of querying, marking entries as nullified, and moving to an adjacent entry as determined by \Cref{cor:core_movement}.
Upon exiting the lower-left quadrant of $B$ (i.e. when the current row is $i \leq m/2$ and/or the current column is $j> m/2$), at least one of the upper-left and lower-right quadrants of $B$ will have been completely marked as nullified.
\end{proposition}
\begin{proof}
Without loss of generality, assume that \sword/ exits the lower-left quadrant to the right. By \Cref{cor:core_movement},  the entries $B_{j,j},\ldots,B_{m/2,j}$ have been marked nullified for each $1\leq j\leq m/2$. Additionally, entries $B_{i,j}$ with $i < j$ are nullified by \Cref{lem:upper_tri}. Thus, entries $B_{i,j}$ for all $1\leq i\leq m/2$ and $1\leq j\leq m/2$ are nullified.
\end{proof}

\Cref{fig:swordfish_big} in the \Cref{appendix:sword} shows an example of the state of \sword/ after one stage; we also refer the reader to \Cref{appendix:sword} for a full description of the \sword/ algorithm.

\subsection{Query Complexity Analysis}
Once the (at most) two subproblems of size $\frac{n}{2} \times \frac{n}{2}$ of a stage of \sword/ have been solved, resulting in two PSNE candidates, we can eliminate at least one of the candidates with a single additional query as follows.
\begin{corollary}[Eliminating a PSNE candidate]\label{cor:2x2elim}
Consider a submatrix $M\in\mathbb{R}^{2\times 2}$ of $A$ such that the diagonal entries are the PSNE candidates and $M_{1,1}\leq M_{2,2}$.
Via \Cref{cor:core_movement}, by querying the entry $M_{2,1}$ we can mark at least one of $M_{1,1}$ and $M_{2,2}$ as nullified.
\end{corollary} 
% \begin{proof}
% % If $B_{i_2,j_1}\leq B_{i_1,j_1}$ then $(i_2,j_2)$ is not the unique PSNE as $B_{i_2,j_2}\geq B_{i_1,j_1}\geq B_{i_2,j_1}$ which violates \eqref{eq:strict_gaps}.
% % If $B_{i_2,j_1}\geq B_{i_1,j_1}$ then $(i_1,j_1)$ is not the unique PSNE as \eqref{eq:strict_gaps} is again violated.
% \end{proof}

Now, let us define $s(n)$ to be the number of queries required by \sword/ for an $n\times n$ matrix. \sword/ requires at most 
\[
s(n)\leq n + (n-1)+2s(n/2)+1 = 2n + 2s(n/2)
\]
queries, due to the diagonal queries, the lower-left quadrant query path, the two subproblems of size $n/2$, and the comparison of two subproblem points, respectively.
Solving this recurrence with $s(1)=1$ gives \[s(n)\leq 2n\log{n}+n\]

Thus, by \cref{eq:strict_gaps} and \Cref{Unique-PSNE}, \sword/ finds the unique PSNE with $\bigO(n\log n)$ queries.
However, there are many modifications that can significantly speed up \sword/ in practice; see Appendix \ref{appendix:sword} for detailed experiments and a slightly more refined complexity analysis.

==> swordfish_experiments.tex <==
\subsection{Experimental results}
Given the sample complexity bound in \Cref{eq:sword_compl_bound}, there are many optimizations that can be made to \sword/ that considerably reduce the number of queries required in practice.
Below, we list some of these optimizations (roughly) in order of effectiveness; though this is certainly not an exhaustive list.
Each optimization is a flag that can be toggled in the Python \sword/ implementation available at \url{https://github.com/QueryEfficientSODA2024/swordfish}.
\begin{itemize}
    \item \texttt{brute\_force}: Before executing \cref{ln:bruteforce}, if the number of remaining non-nullified entries in $B$ is less than some number $b(n)$, query each non-nullified entry and return the PSNE, if it exists.
    Here, $b(n)$ can be a constant, a function of the current submatrix size, or a function of the original matrix size.
    We conjecture that correctly choosing $b(n)$ may be necessary to reduce the theoretical query complexity below $\bigO(n\log n).$
    \item \texttt{quick\_mark}: Before entering the loop in \cref{ln:quickmove}, mark all possible entries of $B$ that can be nullified by previous queries as nullified. 
    This optimization reduces queries in the lower-left quadrant subproblems, as the previous query path gets ``scrambled'' once that quadrant gets diagonally sorted, and entries on the path are thereby able to nullify new entries.
    \item \texttt{recycle}: for a lower-left quadrant subproblem, before diagonally sorting in \cref{ln:bruteforce}, construct a partial diagonal from the parent problem's already-queried entries; this allows for fewer than $n$ new queries to construct a diagonal to be sorted.
    Computing this partial diagonal requires computing the \textit{maximum bipartite matching} of the graph induced by the queried entries of $B$.
    We do so using the Hopcroft–Karp algorithm \citep{hopcroft52Algorithm1973}, available in the \texttt{scipy.sparse} submodule.
    \item \texttt{quick\_move}: in \cref{ln:quickmove}, immediately move without querying another entry, if possible; i.e., if there are $n/2$ nullified entries (via earlier queries) at the beginning of the column or end of the row. 
\end{itemize}
In order to fairly compare these optimizations, we use the following two metrics to measure queries of the input matrix.
\begin{itemize}
    \item \textbf{unique queries}: how many unique entries of $A$ were queried by \sword/.
    \item \textbf{attempted queries}: how many times \sword/ queried an entry (or would have queried an entry) from $A$.
    In other words, these are queries that would have been made, given that the previous history of queries was unavailable (but not necessarily the knowledge of nullified entries).
    For example, the \texttt{recycle} optimization reduces unique queries, but is not (generally) guaranteed to reduce attempted queries, as it requires knowledge of the previous query path.
    The attempted queries metric is useful as it is more indicative of which optimizations may be mathematically proven to be effective, as reasoning about specific queries during the algorithm is challenging.
\end{itemize}

To illustrate the effectiveness of these optimizations in practice, we ran \sword/ against the following 4 problem classes:
\begin{itemize}
    \item \texttt{centered}: An entry is chosen uniformly at random as the Nash equilibrium, with value $V\sim\mathrm{Unif}([1/3, 2/3])$.
    The remaining row and column entries are then drawn i.i.d. from $\mathrm{Unif}([V,1])$ and $\mathrm{Unif}([0,V])$, respectively.
    \item \texttt{skewed}: As above, except we now draw $V\sim\mathrm{Unif}([0, 1/3] \cup [2/3, 1])$.
    \item \texttt{binary}: An entry is chosen uniformly at random as the Nash equilibrium, and assigned value $1/2$.
    Its row and column entries are filled with $1$s and $0$s, respectively, and the rest of the matrix is drawn i.i.d. from $\{0,1\}$.
    \item \texttt{curved} Each entry $(i, j)$ is initially set proportional to $5i + j$ and then perturbed with i.i.d. noise.
    A Nash row $\istar$ is selected from the last $n/2$ rows, and the column $(\jstar)$ corresponding to its minimum is then scaled to make $(\istar, \jstar)$ a PSNE.
\end{itemize}

Below, \Cref{fig:sword_opts} shows the effectiveness of each optimization on the \texttt{random\_centered} problem type, where we normalize the query complexity to the recurrence bound \eqref{eq:sword_compl_bound}.
Using the \texttt{brute\_force} optimization alone reduces the unique queries to below 50\% of the bound \eqref{eq:sword_compl_bound} for $n=2^{10}$.
\begin{figure}[ht!]
\centering
\includesvg[width=0.98\textwidth]{graphics/swordfish_all_opts_comparison.svg}
\caption{``Boxen plot'' of the effectiveness of different \sword/ optimizations for \texttt{random\_centered} matrices. For each $n$, each algorithm was run on the same $200$ input matrices. The \texttt{brute\_force} optimization uses $b(n)=2\log n$.}
\label{fig:sword_opts}
\end{figure}

In \Cref{fig:sword_grid} we demonstrate the effect of enabling all 4 optimizations, run against all 4 problem types.
\begin{figure}[ht!]
\centering
\includesvg[width=\textwidth]{graphics/swordfish_all_types_comparison.svg}
\caption{``Boxen plot'' of the effectiveness of combined \sword/ optimizations across different problem types. For each problem type and for each $n$, each algorithm was run on the same $500$ input matrices.}
\label{fig:sword_grid}
\end{figure}
In contrast to \Cref{fig:sword_opts}, enabling all optimizations further reduces unique queries on the \texttt{random\_centered} problem type to under 35\% of the bound \eqref{eq:sword_compl_bound} for $n=2^{10}$.
These figures suggest that it may be able to reduce the proven query complexity of \sword/ or related algorithms to $O(n)$ or $O(n \log(\log n))$, through better algorithm design and/or a more refined analysis.


==> swordfish_new.tex <==
\section{An \texorpdfstring{$\bigO(n)$}{O(n)} Deterministic Algorithm to Find the Unique PSNE}\label{sec:deterministic}

In this section, we return to the setting in which  the input matrix $A\in\bbR^{n\times n}$ has a unique PSNE $(\istar,\jstar)$, and we
detail \sword/, which has the following guarantee. 
\begin{theorem}
    There is a deterministic algorithm called \sword/ that identifies the unique PSNE $(\istar,\jstar)$ after querying at most $3n-2$ entries from the input matrix $A$.
\end{theorem}
%\subsection{\sword/ in theory}
\noindent The salient feature of  \textsc{Swordfish} is its adaptivity: it limits querying entries of $A$ that can be proven to not be the unique PSNE.
By \Cref{Nash-Shapley-lemma}, the PSNE has positive row and column gaps. That is, 
% \begin{equation}
% A_{(1),\jstar}\leq \ldots \leq A_{(n-1),\jstar}< A_{(n),\jstar}=A_{\istar,\jstar} = A_{\istar,(1)} < A_{\istar,(2)} \leq \ldots \leq A_{\istar,(n)} . \label{eq:strict_gaps}
% \end{equation}
\begin{equation}
A_{i,\jstar}< A_{\istar,\jstar} < A_{\istar,j}\quad \forall i\in [n]\setminus\{\istar\},\: j\in[n]\setminus\{\jstar\} . \label{eq:strict_gaps}
\end{equation}

\begin{definition}
We call an entry $A_{\widehat i,\widehat j}$ \textbf{nullified} by entries $A_{\widehat i,\ell}$ and $A_{k,\widehat  j}$ where $(\widehat  i,\ell)\neq (k,\widehat  j)$ if the two entries jointly contradict \eqref{eq:strict_gaps} for $(\istar,\jstar)=(\widehat i,\widehat j)$, i.e. if $A_{\widehat  i,\ell}\leq A_{k,\widehat j}$ holds.
A nullified entry cannot be the unique PSNE of the matrix $A$.
\end{definition}

\sword/ has two phases. In the first phase, \sword/ proceeds in an iterative fashion as follows. We maintain a set $\calS$ of potential PSNE candidates. At the start of each iteration $1\leq k<n$, we are given a sub-matrix of $A$ called $B_k\in\mathbb{R}^{n-k+1\times n-k+1}$ whose all diagonal entries are queried. During the iteration $k$, we nullify $2(n-k)-1$ entries of $B_k$, add two entries to $\calS$, query one additional element of $B_k$ and create a sub-matrix of $B_k$ called $B_{k+1}\in\mathbb{R}^{n-k\times n-k}$ whose all diagonal entries are queried. $B_{k+1}$ is then used by \sword/ in the iteration $k+1$. Before the start of the first iteration, we set $\calS=\emptyset$ and query all the diagonal entries of $B_1=A$ and then use it in the first iteration. In the iteration $n$, we add the only entry of $B_{n}$ to $\calS$.

We now describe the details of an iteration $k<n$. Consider $\widehat i\in \argmin_{i}(B_{k})_{i,i}$ and $\widehat j\in \argmax_{j}(B_{k})_{j,j}$, that are the indices corresponding to the lowest and highest diagonal entry. Now for all $j\neq \widehat i$, $(B_{k})_{\widehat i, j}$ is nullified by $(B_{k})_{\widehat i, \widehat i}$ and $(B_{k})_{j,j}$ since if $(\widehat{i},j)$ were the PSNE we would have $B_{j,j} < B_{\widehat{i},j} < B_{\widehat{i},\widehat{i}}$, but in fact we have $(B_{k})_{\widehat i, \widehat i}\leq (B_{k})_{j,j}$, a contradiction. Similarly for all $i\neq \widehat j$, $(B_{k})_{i, \widehat j}$ is nullified by $(B_{k})_{\widehat j, \widehat j}$ and $(B_{k})_{i,i}$ as $(B_{k})_{i, i}\leq (B_{k})_{\widehat j,\widehat j}$. We add the entries $(B_{k})_{\widehat i, \widehat i}$ and $(B_{k})_{\widehat j, \widehat j}$ to $\calS$. Next we query the entry $(B_k)_{\widehat j, \widehat i}$. Observe that $(B_k)_{\widehat j, \widehat i}$ is not nullified in the process above.  Now create a sub-matrix $B_{k+1}$ of $B_k$ by first removing the row $\widehat i$ and the column $\widehat j$ from $B_k$ and then rearranging the rows and columns so that the queried entries of $B_{k+1}$ lie on the diagonal. 

Observe that for all $1\leq k<n$, the elements in $B_{k}$ that are not part of $B_{k+1}$ are either nullified or added to $\calS$. Moreover, recall that the only entry of $B_{n}$ is added to $\calS$. Hence, all entries of $A$ are either nullified or added to $\calS$. Note that the PSNE $(\istar,\jstar)$ can not be nullified. Hence, it must be part of $\calS$. 

Now given the set $\calS$ of entries in $A$, \sword/ aims to find the PSNE $(\istar,\jstar)$ of $A$ in its second phase. First we perform some pre-processing of $A$. 
If $\calS$ contains multiple elements from a row, we just retain at most one element which is equal to the one achieving the unique minimum of those queried, if it exists, and remove rest from $\calS$ as they are nullified (as $A_{\istar,\jstar} < A_{\istar,j}$ for $j \neq \jstar$). 
Similarly, if $\calS$ contains multiple elements from a column, we only maintain the unique maximizer, if it exists, and discard all others from $\calS$ as they are nullified (as $A_{\istar,\jstar} > A_{i,\jstar}$ for $i \neq \istar$). 
% Similarly if there are more than one queried elements in a column, we only retain the unique highest queried element, if it exists, and discard rest of the queried elements from $\calS$ as they are nullified. 
Now we are left with at most one element in each row and column of $A$ and $|\calS|\leq n$. Now let us reorder the rows and columns so that the entries in $\calS$ become the diagonal entries $A_{1,1},A_{2,2},\ldots,A_{s,s}$ where $s=|\calS|$. Let us also assume that $A_{1,1}\leq A_{2,2}\leq \ldots,A_{s,s}$. Now \sword/ proceeds in an iterative fashion as follows. In each iteration, we maintain $\widehat i, \widehat j$ such that $\widehat j\leq \widehat i$. Before the start of the first iteration, we set $\widehat i=2$ and $\widehat j=1$. Now in an iteration $k$, we query the entry $A_{\widehat i,\widehat j}$. If $A_{\widehat i,\widehat j}\leq A_{\widehat i,\widehat i}$ then $A_{\widehat i,\widehat i}$ is nullified and we remove it from $\calS$. Similarly, if $A_{\widehat i,\widehat j}\geq A_{\widehat j,\widehat j}$ then $A_{\widehat j,\widehat j}$ is nullified and we remove it from $\calS$. As $A_{\widehat j,\widehat j}\leq A_{\widehat i, \widehat i}$, at least one of $A_{\widehat i,\widehat i}$ and $A_{\widehat j,\widehat j}$ is nullified. If only $A_{\widehat i,\widehat i}$ was nullified then we increment $\widehat i$ by one. Similarly if only $A_{\widehat j,\widehat j}$ was nullified then we set $\widehat j=\widehat i$ and increment $\widehat i$ by one. If both $A_{\widehat i,\widehat i}$ and $A_{\widehat j,\widehat j}$ were nullified then we set $\widehat j=\widehat i+1$ and increment $\widehat i$ by two. We then proceed to the next iteration $k+1$. We terminate the procedure when there is only one element left in $\calS$ and return that element as the PSNE of $A$. Note that the PSNE of $A$ is never removed from $\calS$ as it is never nullified. Hence, we indeed return the PSNE of $A$.   

The total number of queries in the first phase is $2n-1$ as we query $n$ entries before the first iteration and then query one entry in each of the first $n-1$ iterations. The total number of queries in the second phase is at most $n-1$ as the number of iterations is at most $n-1$ and in each iteration we query one entry and remove at least one entry from $\calS$. Hence, the query complexity of \sword/ is at most $3n-2$. \sword/ is formally described in \Cref{appendix:sword}.

